Classification with unknown class-conditional label noise on non-compact feature spaces

We investigate the problem of classification in the presence of unknown class-conditional label noise in which the labels observed by the learner have been corrupted with some unknown class dependent probability. In order to obtain finite sample rates, previous approaches to classification with unknown class-conditional label noise have required that the regression function is close to its extrema on sets of large measure. We shall consider this problem in the setting of non-compact metric spaces, where the regression function need not attain its extrema. In this setting we determine the minimax optimal learning rates (up to logarithmic factors). The rate displays interesting threshold behaviour: When the regression function approaches its extrema at a sufficient rate, the optimal learning rates are of the same order as those obtained in the label-noise free setting. If the regression function approaches its extrema more gradually then classification performance necessarily degrades. In addition, we present an adaptive algorithm which attains these rates without prior knowledge of either the distributional parameters or the local density. This identifies for the first time a scenario in which finite sample rates are achievable in the label noise setting, but they differ from the optimal rates without label noise.

==> Archive/boundsForAsymmetricLabelNoise.tex <==


\subsection{A simple method for uniform smoothness}\label{mainBoundForUniformSmoothnessSec}

\begin{algorithm}[htbp]
%\floatconts
%{alg:KNNInd}
 {\caption{A k nearest neighbour method for label noise\label{KNNForLabelNoiseUniformCaseAlgo}}}
{ 
 \begin{enumerate}
     \item Compute the nearest neighbour estimate $\noisy[{\est[\regressionFunction]}](x) =\KNNLepskiEstBase{{(\noisy[\regressionFunction])}}{n}{\delta^2/3}(x)$ with sample $\noisy[\sample]$;
     \item Compute $\estProbFlipZeroToOne = 1-{\empiricalMaximumBase{{1-\noisy[\regressionFunction]}}{n}{\delta/3}}$ and $\estProbFlipOneToZero = 1-\empiricalMaximumBase{{\noisy[\regressionFunction]}}{n}{\delta/3}$;
     \item Let $\est[\classifier]_{n,\delta}(x):= \one\left\lbrace \noisy[{\est[\regressionFunction]}](x) \geq 1/2 \cdot \left(1+\estProbFlipZeroToOne-\estProbFlipOneToZero\right) \right\rbrace$.
     \end{enumerate}
 }
\end{algorithm}


In addition to Assumption \ref{rangeAssumption} we shall make the following assumptions.
\begin{assumption}[Uniform smoothness]\label{regressionFunctionIsUniformlySmoothAssumption} The regression function $\regressionFunction$ is uniformly measure-smooth with exponent $\measureSmoothnessExponent$ and constant $\measureSmoothnessConstant \geq 1$.
\end{assumption}
We shall also use Tysbakov's margin assumption \cite{tsybakov2004optimal}.
\begin{restatable}[Margin condition]{assumption}{marginAssumption}\label{marginAssumption} There exists $\marginExponent\geq 0$ and $\marginConstant \geq 1$ such that for all $\xi>0$ we have
\begin{align*}
\marginalDistribution\left( \left\lbrace x \in \X: 0< \left|\regressionFunction(x)-\frac{1}{2}\right| <\xi \right\rbrace \right) \leq \marginConstant \cdot \xi^{\marginExponent}.
\end{align*}
\end{restatable}
Note that Assumption \ref{marginAssumption} always holds with $\marginExponent=0$ and $\marginConstant = 1$.

\begin{theorem}\label{riskBoundForUniformSmoothnessThm} Suppose that Assumption \ref{rangeAssumption} holds, Assumption \ref{regressionFunctionIsUniformlySmoothAssumption} holds with exponent $\measureSmoothnessExponent>0$ and constant $\measureSmoothnessConstant\geq 1$, and Assumption \ref{marginAssumption} holds with constant $\marginExponent\geq 0$ and $\marginConstant\geq 1$. Take any $n \in \N$, $\delta \in \left(0,1\right)$ and suppose we have  $\noisySample = \left\lbrace \left(X_i,\noisy[Y]_i\right)\right\rbrace_{i \in [n]}$ with $\left(X_i,\noisy[Y]_i\right) \sim \noisy[\Prob]$. Let $\est[\classifier]_{n,\delta}$ be the classifier introduced in Algorithm \ref{KNNForLabelNoiseUniformCaseAlgo}. With probability at least $1-\delta$ over $\noisy[\sample]$, 
\begin{align}\label{riskBoundForUniformSmoothnessThmEq}
\risk\left(\est[\classifier]_{n,\delta}\right) \leq \risk\left(\oracle\right)+\marginConstant \cdot \left(\frac{120\cdot \measureSmoothnessConstant}{\left(1-\probFlipZeroToOne-\probFlipOneToZero\right)^2}\right)^{\marginExponent+1} \cdot \left( \frac{\log(3n/\delta)}{n}\right)^{\frac{\measureSmoothnessExponent\cdot(\marginExponent+1)}{2\measureSmoothnessExponent+1}}+\delta.
\end{align}
\end{theorem}
\newcommand{\goodDeltaSet}{\mathcal{G}_{\delta}}
\newcommand{\smallErrors}{\zeta(n,\delta)}
\begin{proof} For the purpose of this proof we write $\smallErrors:=14\sqrt{2} \cdot \measureSmoothnessConstant \cdot \left( \frac{\log(3n/2\delta)}{n}\right)^{\frac{\measureSmoothnessExponent}{2\measureSmoothnessExponent+1}}$ and define 
\[\goodDeltaSet := \left\lbrace x \in \suppMarginalDistribution: \left|\noisy[{\est[\regressionFunction]}](x)-\noisy[\regressionFunction](x)\right|\leq  \smallErrors \right\rbrace.\]
By Corollary \ref{KNNPointwiseBoundLepskiChoiceKThm} for each $x \in \suppMarginalDistribution$ the following holds with probability at least $1-\delta^2/3$,
\begin{align*}
\left|\noisy[{\est[\regressionFunction]}](x)-\noisy[\regressionFunction](x)\right|&\leq  6\sqrt{2}\cdot \localMeasureSmoothnessFactor[x]^{\frac{1}{2\measureSmoothnessExponent+1}} \cdot \left( \frac{\log(3n/2(\delta^2/3))}{n}\right)^{\frac{\measureSmoothnessExponent}{2\measureSmoothnessExponent+1}}\\
&\leq 12 \cdot \measureSmoothnessConstant^{\frac{1}{2\measureSmoothnessExponent+1}} \cdot \left( \frac{\log(3n/\delta)}{n}\right)^{\frac{\measureSmoothnessExponent}{2\measureSmoothnessExponent+1}}\leq \smallErrors.
\end{align*}
Hence, for each $x \in \X$, we have $x \in \goodDeltaSet$ with probability at least $1-\delta^2/3$, so by Fubini's theorem we have
\begin{align*}
\E_{\sample}\left[\Prob\left[\X\backslash \goodDeltaSet\right]\right] = \E_{\sample}\left[\E_{(X,Y) \sim \Prob}\left[\one\left\lbrace X \notin \goodDeltaSet\right\rbrace \right]\right] =\E_{(X,Y) \sim \Prob}\left[\E_{\sample}\left[\one\left\lbrace X \notin \goodDeltaSet\right\rbrace \right]\right]\leq \delta^2/3.      
\end{align*}
Hence, by Markov's inequality we have $\Prob\left[\X\backslash \goodDeltaSet\right]\leq \delta$ with probability at least $1-\delta/3$. Moreover, by Theorem \ref{NaiveMaxBoundThm} the following holds with probability at least $1-\delta/3$ we have
\begin{align*}
\left|\estProbFlipZeroToOne -\estProbFlipZeroToOne\right|\leq  14\cdot \measureSmoothnessConstant \cdot \left( \frac{\log(3n/(\delta/3))}{n}\right)^{\frac{\measureSmoothnessExponent}{2\measureSmoothnessExponent+1}} \leq \smallErrors.    
\end{align*}
Similarly, with  probability at least $1-\delta/3$ we have $\left|\estProbFlipOneToZero -\estProbFlipOneToZero\right|\leq \smallErrors$. Thus, by the union bound, with probability at least $1-\delta$, we have $\Prob\left[\X\backslash\goodDeltaSet\right]\leq \delta$ and $\max\left\lbrace \left|\estProbFlipZeroToOne -\estProbFlipZeroToOne\right| ,\left|\estProbFlipOneToZero -\estProbFlipOneToZero\right|\right\rbrace \leq \smallErrors$. Hence, it suffices to assume that $\Prob\left[\X\backslash\goodDeltaSet\right]\leq \delta$ and $\max\left\lbrace \left|\estProbFlipZeroToOne -\estProbFlipZeroToOne\right| ,\left|\estProbFlipOneToZero -\estProbFlipOneToZero\right|\right\rbrace \leq \smallErrors$ holds and deduce (\ref{riskBoundForUniformSmoothnessThmEq}). Observe that we can rewrite $\est[\classifier]_{n,\delta}:\X\rightarrow \Y$ as $\est[\classifier]_{n,\delta}(x)=\one\left\lbrace \est{\regressionFunction}(x)\geq 1/2\right\rbrace$, where $\est[\regressionFunction](x):= \left(\noisy[{\est[\regressionFunction]}](x)-\estProbFlipZeroToOne\right)/\left(1-\estProbFlipZeroToOne-\estProbFlipOneToZero\right)$. By Lemma \ref{elementaryRatioLemma} for all $x \in \goodDeltaSet$ we have
\begin{align*}
\left| \est[\regressionFunction](x)-\regressionFunction(x)\right| &\leq 6 \cdot \left(1-\probFlipZeroToOne-\probFlipOneToZero\right)^{-2} \cdot \max\left\lbrace \left| \estNoisyRegressionFunction(x) - \noisyRegressionFunction(x)\right|, \left| \estProbFlipZeroToOne-\probFlipZeroToOne \right|, \left| \estProbFlipOneToZero-\probFlipOneToZero \right| \right\rbrace\\ &\leq  6 \cdot \left(1-\probFlipZeroToOne-\probFlipOneToZero\right)^{-2} \cdot \smallErrors.
\end{align*}
Hence, given any $x \in \X$ with $\est[\classifier]_{n,\delta}(x)\neq \oracle(x)=\one\left\lbrace \regressionFunction(x)\geq 1/2\right\rbrace$ we must have $\left|\regressionFunction(x)-1/2\right|\leq 6 \cdot \left(1-\probFlipZeroToOne-\probFlipOneToZero\right)^{-2} \cdot \smallErrors$. Hence, by Assumption \ref{marginAssumption}, with probability at least $1-\delta$, we have
\begin{align*}
\risk\left(\est[\classifier]_{n,\delta}\right) -\risk\left(\oracle\right) & = \int_{\X} \left|\regressionFunction(x)-\frac{1}{2}\right|\cdot \one\left\lbrace \est[\classifier]_{n,\delta}(x)\neq \oracle(x)\right\rbrace d\marginalDistribution(x)\\
&\leq \int_{\goodDeltaSet} \left|\regressionFunction(x)-\frac{1}{2}\right|\cdot \one\left\lbrace \est[\classifier]_{n,\delta}(x)\neq \oracle(x)\right\rbrace d\marginalDistribution(x)+\Prob\left[\X\backslash \goodDeltaSet\right]\\
&\leq  \int_{\X} \left|\regressionFunction(x)-\frac{1}{2}\right|\cdot \one\left\lbrace  \left|\regressionFunction(x)-\frac{1}{2}\right| \leq \frac{ 6 \cdot \smallErrors}{ \left(1-\probFlipZeroToOne-\probFlipOneToZero\right)^2} \right\rbrace d\marginalDistribution(x)+\delta\\
&\leq \marginConstant \cdot \left(\frac{6 \cdot \smallErrors}{ \left(1-\probFlipZeroToOne-\probFlipOneToZero\right)^2} \right)^{\marginExponent+1} +\delta\\
& = \marginConstant \cdot \left(\frac{120 \cdot \measureSmoothnessConstant}{\left(1-\probFlipZeroToOne-\probFlipOneToZero\right)^2}\right)^{\marginExponent+1} \cdot \left( \frac{\log(3n/\delta)}{n}\right)^{\frac{\measureSmoothnessExponent\cdot(\marginExponent+1)}{2\measureSmoothnessExponent+1}}+\delta.
\end{align*}
This completes the proof of the theorem.
\end{proof}



\subsection{A method for non-uniform smoothness}\label{mainBoundForNonUniformSmoothnessSec}

We shall now deal with the more challenging setting in which uniform smoothness is not assumed.

\begin{algorithm}[htbp]
 {\caption{A robust k nearest neighbour method for label noise\label{KNNForLabelNoiseNonUniformCaseAlgo}}}
{ 
 \begin{enumerate}
     \item Compute the nearest neighbour estimate $\noisy[{\est[\regressionFunction]}](x) =\KNNLepskiEstBase{{(\noisy[\regressionFunction])}}{n}{\delta^2/3}(x)$ with sample $\noisy[\sample]$;
     \item Compute $\estProbFlipZeroToOne = 1-{\maxEstNDeltaBase{{1-\noisy[\regressionFunction]}}{n}{\delta/3}}$ and $\estProbFlipOneToZero = 1-\maxEstNDeltaBase{{\noisy[\regressionFunction]}}{n}{\delta/3}$;
     \item Let $\est[\classifier]_{n,\delta}(x):= \one\left\lbrace \noisy[{\est[\regressionFunction]}](x) \geq 1/2 \cdot \left(1+\estProbFlipZeroToOne-\estProbFlipOneToZero\right) \right\rbrace$.
     \end{enumerate}
 }
\end{algorithm}

To bound the performance of Algorithm \ref{KNNForLabelNoiseNonUniformCaseAlgo} we shall make the following assumptions.

\begin{assumption}[Measure smoothness]\label{regressionFunctionMeasureSmoothAssumption} The regression is measure smooth with exponent $\measureSmoothnessExponent>0$ and multiplier function $\localMeasureSmoothnessFactorFunction:\X\rightarrow [1,\infty)$.
\end{assumption}

\marginAssumption*

\begin{assumption}[Polynomial tails]\label{tailsAssumption} There exists and exponent $\tailsExponent>0$ and a constant $\tailsConstant\geq 1$ such that for all $t>0$ we have $\marginalDistribution\left(\left\lbrace x \in \X: \localMeasureSmoothnessFactor[x]>t \right\rbrace\right) \leq \tailsConstant \cdot t^{-\tailsExponent}$.
\end{assumption}


\begin{assumption}[Fast limits condition]\label{fastLimitsForRegressionFunctionAssumption} There exists an exponent $\fastLimitsExponent>0$ and constants $\fastLimitsConstant\geq 1$ and $\fastLimitsLowerBoundConstant>0$ such that for all $t \geq \fastLimitsLowerBoundConstant$ we have $\inf_{x \in \suppMarginalDistribution}\left\lbrace \regressionFunction(x): \localMeasureSmoothnessFactor[x]\leq t \right\rbrace \leq \fastLimitsConstant\cdot t^{-\fastLimitsExponent}$ and
$\sup_{x \in \suppMarginalDistribution}\left\lbrace \regressionFunction(x): \localMeasureSmoothnessFactor[x]\leq t \right\rbrace \geq 1-\fastLimitsConstant\cdot t^{-\fastLimitsExponent}$.
\end{assumption}

\newcommand{\mainExponentForUnboundedRiskBoundThm}{\frac{\measureSmoothnessExponent \left(\fastLimitsExponent\wedge(\tailsExponent/\marginExponent)\right)(\marginExponent+1)}{1+\left(\fastLimitsExponent\wedge(\tailsExponent/\marginExponent)\right)(2\measureSmoothnessExponent+1)}}
\begin{samepage}
\begin{theorem}\label{riskBoundForNonUniformSmoothnessThm} Suppose that Assumption \ref{rangeAssumption} holds, Assumption \ref{regressionFunctionMeasureSmoothAssumption} holds with exponent $\measureSmoothnessExponent>0$ and multiplier function $\localMeasureSmoothnessFactorFunction:\X \rightarrow [1,\infty)$, Assumption \ref{marginAssumption} holds with exponent $\marginExponent\geq 0$ and constant $\marginConstant\geq 1$, Assumption \ref{tailsAssumption} holds with exponent $\tailsExponent>0$ and constant $\tailsConstant \geq 1$ and Assumption \ref{fastLimitsForRegressionFunctionAssumption} holds with exponent $\fastLimitsExponent>0$ and constants $\fastLimitsConstant,\fastLimitsLowerBoundConstant\geq 0$. Suppose further that $\tailsExponent(2\measureSmoothnessExponent+1)>1$ and let $C(\marginExponent,\fastLimitsExponent, \tailsExponent, \marginalDistribution):=\marginConstant\cdot \left(26\left(\fastLimitsConstant+2^4\cdot \doublingConstant[\marginalDistribution]\right)\right)^{\marginExponent+1}\cdot\left(1-2^{1-\tailsExponent(2\measureSmoothnessExponent+1)}\right)^{-1}$. Take $\delta \in \left(0,1\right)$ and $n \in \N$ sufficiently large that $n/\log(3n/\delta) \geq \fastLimitsLowerBoundConstant^{\frac{1+\fastLimitsExponent(2\measureSmoothnessExponent+1)}{\measureSmoothnessExponent}}$. With probability at least $1-\delta$ we have
\begin{align}\label{riskBoundForNonUniformSmoothnessThmEq}
\risk\left(\est[\classifier]_{n,\delta}\right)-\risk\left(\oracle\right) \leq \begin{cases} C(\marginExponent,\fastLimitsExponent, \tailsExponent, \marginalDistribution) \cdot\left(1-\probFlipZeroToOne-\probFlipOneToZero\right)^{-2(\marginExponent+1)}\cdot\left(\frac{\log(3n/\delta)}{n}\right)^{\frac{\measureSmoothnessExponent  \fastLimitsExponent(\marginExponent+1)}{1+\fastLimitsExponent(2\measureSmoothnessExponent+1)}}+\delta & \text{ when }\marginExponent \cdot \fastLimitsExponent < \tailsExponent\\
 C(\marginExponent,\fastLimitsExponent, \tailsExponent, \marginalDistribution) \cdot\left(1-\probFlipZeroToOne-\probFlipOneToZero\right)^{-2(\marginExponent+1)}\cdot\left(\frac{\log(3n/\delta)}{n}\right)^{\frac{\measureSmoothnessExponent \tailsExponent(\marginExponent+1)}{\marginExponent+\tailsExponent(2\measureSmoothnessExponent+1)}}+\delta &\text{ otherwise.}
\end{cases}
\end{align}
\end{theorem}
\end{samepage}


\renewcommand{\goodDeltaSet}{\mathcal{G}_{\delta}}
\newcommand{\goodDeltaSetByInd}[1][j]{\mathcal{G}_{\delta}^{#1}}
\newcommand{\smallErrorsByX}[1][x]{\zeta(#1,n,\delta)}
\newcommand{\smallErrorsByInd}[1][j]{\zeta_{#1}(n,\delta)}
\newcommand{\epsilonByNDelta}{\epsilon(n,\delta)}
\newcommand{\wellBehavedLocalMultiplierExponent}{\kappa_0}
\newcommand{\localConstantT}{K}
\newcommand{\excessErrorOnGoodDeltaSetByInd}[1][j]{\mathcal{E}_{\delta}^{#1}}


\begin{proof} The proof begins in a similar way to the proof of Theorem \ref{riskBoundForUniformSmoothnessThm}. The main difference is that as there is no uniform bound on $\localMeasureSmoothnessFactor$ we must explicitly take its local value into account. For the purpose of this proof we write $\epsilonByNDelta:= \log(3n/\delta)/n$. Note that we can assume, without loss of generality, that $\epsilonByNDelta\leq 1$, since the conclusion of the theorem is trivial if $\epsilonByNDelta> 1$. In addition we let $\smallErrorsByX:=\sqrt{2}\left(\fastLimitsConstant+2^4 \cdot \doublingConstant[\marginalDistribution]\right) \cdot \max\left\lbrace \localMeasureSmoothnessFactor^{\frac{1}{2\measureSmoothnessExponent+1}}\cdot \epsilonByNDelta^{\frac{\measureSmoothnessExponent}{2\measureSmoothnessExponent+1}}, \epsilonByNDelta^{\frac{\fastLimitsExponent \measureSmoothnessExponent}{1+\fastLimitsExponent(2\measureSmoothnessExponent+1)}} \right\rbrace$ and define 
\[\goodDeltaSet := \left\lbrace x \in \suppMarginalDistribution: \left|\noisy[{\est[\regressionFunction]}](x)-\noisy[\regressionFunction](x)\right|\leq  \smallErrorsByX \right\rbrace.\]
By Corollary \ref{KNNPointwiseBoundLepskiChoiceKThm} combined with Assumption \ref{regressionFunctionMeasureSmoothAssumption} we see that for each $x \in \suppMarginalDistribution$ the following holds with probability at least $1-\delta^2/3$,
\begin{align*}
\left|\noisy[{\est[\regressionFunction]}](x)-\noisy[\regressionFunction](x)\right|&\leq  6\sqrt{2}\cdot \localMeasureSmoothnessFactor[x]^{\frac{1}{2\measureSmoothnessExponent+1}} \cdot \left( \frac{\log(3n/2(\delta^2/3))}{n}\right)^{\frac{\measureSmoothnessExponent}{2\measureSmoothnessExponent+1}}\leq \smallErrorsByX,
\end{align*}
where we have used the fact that $\doublingConstant\geq 1$. Hence, for each $x \in \X$, we have $x \in \goodDeltaSet$ with probability at least $1-\delta^2/3$, so by Fubini's theorem we have
\begin{align*}
\E_{\sample}\left[\Prob\left[\X\backslash \goodDeltaSet\right]\right] = \E_{\sample}\left[\E_{(X,Y) \sim \Prob}\left[\one\left\lbrace X \notin \goodDeltaSet\right\rbrace \right]\right] =\E_{(X,Y) \sim \Prob}\left[\E_{\sample}\left[\one\left\lbrace X \notin \goodDeltaSet\right\rbrace \right]\right]\leq \delta^2/3.      
\end{align*}
Hence, by Markov's inequality we have $\Prob\left[\X\backslash \goodDeltaSet\right]\leq \delta$ with probability at least $1-\delta/3$. Moreover, by Corollary \ref{fastLimitsForRegressionFunctionAssumption} combined with Assumption \ref{fastLimitsForRegressionFunctionAssumption} the following holds with probability at least $1-\delta/3$ we have
\begin{align*}
\left|\estProbFlipZeroToOne -\estProbFlipZeroToOne\right|&\leq \left(\fastLimitsConstant+2^4\cdot \doublingConstant[\marginalDistribution]^{\frac{2\measureSmoothnessExponent}{2\measureSmoothnessExponent+1}}\right) \cdot \left(\frac{\log(2n/(\delta/3))}{n}\right)^{\frac{\fastLimitsExponent \measureSmoothnessExponent}{1+\fastLimitsExponent(2\measureSmoothnessExponent+1)}}\\   
&\leq \sqrt{2}\left(\fastLimitsConstant+2^4\cdot \doublingConstant[\marginalDistribution]\right) \cdot \left(\frac{\log(3n/\delta))}{n}\right)^{\frac{\fastLimitsExponent \measureSmoothnessExponent}{1+\fastLimitsExponent(2\measureSmoothnessExponent+1)}}\leq \inf_{x \in \suppMarginalDistribution}\left\lbrace \smallErrorsByX \right\rbrace.
\end{align*}
Similarly, with  probability at least $1-\delta/3$ we have $\left|\estProbFlipOneToZero -\estProbFlipOneToZero\right|\leq \inf_{x \in \suppMarginalDistribution}\left\lbrace \smallErrorsByX \right\rbrace$. Hence, it suffices to assume that $\Prob\left[\X\backslash\goodDeltaSet\right]\leq \delta$ and $\max\left\lbrace \left|\estProbFlipZeroToOne -\estProbFlipZeroToOne\right| ,\left|\estProbFlipOneToZero -\estProbFlipOneToZero\right|\right\rbrace \leq \inf_{x \in \suppMarginalDistribution}\left\lbrace \smallErrorsByX \right\rbrace$ holds and deduce (\ref{riskBoundForNonUniformSmoothnessThmEq}).




We can rewrite $\est[\classifier]_{n,\delta}:\X\rightarrow \Y$ as $\est[\classifier]_{n,\delta}(x)=\one\left\lbrace \est{\regressionFunction}(x)\geq 1/2\right\rbrace$, where $\est[\regressionFunction](x):= \left(\noisy[{\est[\regressionFunction]}](x)-\estProbFlipZeroToOne\right)/\left(1-\estProbFlipZeroToOne-\estProbFlipOneToZero\right)$. By Lemma \ref{elementaryRatioLemma} for all $x \in \goodDeltaSet$ we have
\begin{align*}
\left| \est[\regressionFunction](x)-\regressionFunction(x)\right| &\leq 6 \cdot \left(1-\probFlipZeroToOne-\probFlipOneToZero\right)^{-2} \cdot \max\left\lbrace \left| \estNoisyRegressionFunction(x) - \noisyRegressionFunction(x)\right|, \left| \estProbFlipZeroToOne-\probFlipZeroToOne \right|, \left| \estProbFlipOneToZero-\probFlipOneToZero \right| \right\rbrace\\ &\leq  6 \cdot \left(1-\probFlipZeroToOne-\probFlipOneToZero\right)^{-2} \cdot \smallErrorsByX.
\end{align*}
We now write $\wellBehavedLocalMultiplierExponent:=\max\left\lbrace \frac{\marginExponent \measureSmoothnessExponent}{\marginExponent+\tailsExponent(2\measureSmoothnessExponent+1)}, \frac{\measureSmoothnessExponent}{1+\fastLimitsExponent(2\measureSmoothnessExponent+1)}\right\rbrace$.  Note that this implies $\frac{(\measureSmoothnessExponent-\wellBehavedLocalMultiplierExponent)(\marginExponent+1)}{2\measureSmoothnessExponent+1}=\mainExponentForUnboundedRiskBoundThm$, where $a\wedge b = \min\{a,b\}$ for $a,b \in \R\cup\{+\infty\}$ and $\tailsExponent/\marginExponent=+\infty$ whenever $\tailsExponent>0$ and $\marginExponent=0$. In addition we define a family of subsets $\left\lbrace \goodDeltaSetByInd[j]\right\rbrace_{j= 0}^{\infty}$ such that $\goodDeltaSet\subseteq \bigcup_{j = 0}^{\infty}\goodDeltaSetByInd[j]$ by $\goodDeltaSetByInd[0]:=\left\lbrace x \in \goodDeltaSet: \localMeasureSmoothnessFactor[x]\leq  \epsilonByNDelta^{-\wellBehavedLocalMultiplierExponent} \right\rbrace$, and for $j\geq 1$,
\begin{align*}
\goodDeltaSetByInd[j]:= \left\lbrace x \in \goodDeltaSet: 2^{(j-1)(2\measureSmoothnessExponent+1)}\cdot  \epsilonByNDelta^{-\wellBehavedLocalMultiplierExponent}\leq \localMeasureSmoothnessFactor[x]\leq 2^{j(2\measureSmoothnessExponent+1)}\cdot  \epsilonByNDelta^{-\wellBehavedLocalMultiplierExponent}\right\rbrace.
\end{align*}
Thus, if we let $\localConstantT:={ 6\sqrt{2}\left(\fastLimitsConstant+2^4 \cdot \doublingConstant[\marginalDistribution]\right)}\cdot {  \left(1-\probFlipZeroToOne-\probFlipOneToZero\right)^{-2}}$ then for each $j\geq 0$ and $x \in \goodDeltaSetByInd[j]$ we have 
\begin{align*}
\left| \est[\regressionFunction](x)-\regressionFunction(x)\right| &\leq  6 \cdot \left(1-\probFlipZeroToOne-\probFlipOneToZero\right)^{-2} \cdot \smallErrorsByX\\
& =  \localConstantT  \cdot \max\left\lbrace \localMeasureSmoothnessFactor^{\frac{1}{2\measureSmoothnessExponent+1}}\cdot \epsilonByNDelta^{\frac{\measureSmoothnessExponent}{2\measureSmoothnessExponent+1}}, \epsilonByNDelta^{\frac{\fastLimitsExponent \measureSmoothnessExponent}{1+\fastLimitsExponent(2\measureSmoothnessExponent+1)}} \right\rbrace\\
& \leq \localConstantT  \cdot \max\left\lbrace \left(2^{j(2\measureSmoothnessExponent+1)}\cdot \epsilonByNDelta^{-\wellBehavedLocalMultiplierExponent}\right)^{\frac{1}{2\measureSmoothnessExponent+1}}\cdot \epsilonByNDelta^{\frac{\measureSmoothnessExponent}{2\measureSmoothnessExponent+1}}, \epsilonByNDelta^{\frac{\fastLimitsExponent \measureSmoothnessExponent}{1+\fastLimitsExponent(2\measureSmoothnessExponent+1)}} \right\rbrace\\
& = 2^j \cdot \localConstantT \cdot \epsilonByNDelta^{\frac{\measureSmoothnessExponent-\wellBehavedLocalMultiplierExponent}{2\measureSmoothnessExponent+1}}.
\end{align*}
Here we use the assumption that $\epsilonByNDelta\leq 1$ and $\wellBehavedLocalMultiplierExponent\geq  \frac{\measureSmoothnessExponent}{1+\fastLimitsExponent(2\measureSmoothnessExponent+1)}$. In particular, this means that if $x \in \goodDeltaSetByInd[j]$ for some $j\geq 0$ and $\est[\classifier]_{n,\delta}(x)\neq \oracle(x)$ then $\left| \regressionFunction(x)-\frac{1}{2}\right|\leq 2^j \cdot \localConstantT \cdot \epsilonByNDelta^{\frac{\measureSmoothnessExponent-\wellBehavedLocalMultiplierExponent}{2\measureSmoothnessExponent+1}}$. For each $j \geq 0$ we let 
\begin{align*}
\excessErrorOnGoodDeltaSetByInd[j]&:=\int_{\goodDeltaSetByInd[j]}\left|\regressionFunction(x)-\frac{1}{2}\right| \cdot \one\left\lbrace \est[\classifier]_{n,\delta}(x)\neq \oracle(x)\right\rbrace d\marginalDistribution(x) \\ &\leq 2^j \cdot \localConstantT \cdot \epsilonByNDelta^{\frac{\measureSmoothnessExponent-\wellBehavedLocalMultiplierExponent}{2\measureSmoothnessExponent+1}} \cdot \marginalDistribution\left(\left\lbrace x \in \goodDeltaSetByInd[j]: 0< \left| \regressionFunction(x)-\frac{1}{2}\right|\leq 2^j \cdot \localConstantT \cdot \epsilonByNDelta^{\frac{\measureSmoothnessExponent-\wellBehavedLocalMultiplierExponent}{2\measureSmoothnessExponent+1}}\right\rbrace \right).
\end{align*}
For $j=0$ we apply Assumption \ref{marginAssumption} to infer that 
\begin{align*}
\marginalDistribution\left(\left\lbrace x \in \goodDeltaSetByInd[0]: 0<\left| \regressionFunction(x)-\frac{1}{2}\right|\leq \localConstantT \cdot \epsilonByNDelta^{\frac{\measureSmoothnessExponent-\wellBehavedLocalMultiplierExponent}{2\measureSmoothnessExponent+1}}\right\rbrace \right)  \leq \marginConstant\cdot \left(\localConstantT \cdot \epsilonByNDelta^{\frac{\measureSmoothnessExponent-\wellBehavedLocalMultiplierExponent}{2\measureSmoothnessExponent+1}} \right)^{\marginExponent}.
\end{align*}
Thus, given the definiton of $\wellBehavedLocalMultiplierExponent$ we have 
\begin{align*}
\excessErrorOnGoodDeltaSetByInd[0] \leq \marginConstant \cdot \localConstantT^{\marginExponent+1}\cdot \epsilonByNDelta^{\frac{(\measureSmoothnessExponent-\wellBehavedLocalMultiplierExponent)(\marginExponent+1)}{2\measureSmoothnessExponent+1}} = \marginConstant \cdot \localConstantT^{\marginExponent+1}\cdot \epsilonByNDelta^{\mainExponentForUnboundedRiskBoundThm}.    
\end{align*}
On the other hand, for $j\geq 1$, by Assumption \ref{tailsAssumption} we have
\begin{align*}
\marginalDistribution\left(\goodDeltaSetByInd[j]\right) \leq \marginalDistribution\left(\left\lbrace x \in \X: \localMeasureSmoothnessFactor[x] \geq 2^{(j-1)(2\measureSmoothnessExponent+1)}\cdot \epsilonByNDelta^{-\wellBehavedLocalMultiplierExponent} \right\rbrace\right) \leq 2^{-(j-1)(2\measureSmoothnessExponent+1)\tailsExponent} \cdot \epsilonByNDelta^{\wellBehavedLocalMultiplierExponent \cdot \tailsExponent}.
\end{align*}
Hence, given that $\wellBehavedLocalMultiplierExponent \geq \frac{\marginExponent \measureSmoothnessExponent}{\marginExponent+\tailsExponent(2\measureSmoothnessExponent+1)}$ and $\epsilonByNDelta \leq 1$, for $j\geq 1$ we have
\begin{align*}
\excessErrorOnGoodDeltaSetByInd[j]&\leq 2\localConstantT\cdot 2^{-(j-1)\left(\tailsExponent(2\measureSmoothnessExponent+1)-1\right)} \cdot \epsilonByNDelta^{\frac{\measureSmoothnessExponent+\wellBehavedLocalMultiplierExponent\left(\tailsExponent(2\measureSmoothnessExponent+1)-1\right)}{2\measureSmoothnessExponent+1}}\\
&\leq 2\localConstantT\cdot 2^{-(j-1)\left(\tailsExponent(2\measureSmoothnessExponent+1)-1\right)} \cdot \epsilonByNDelta^{\frac{(\measureSmoothnessExponent-\wellBehavedLocalMultiplierExponent)(\marginExponent+1)}{2\measureSmoothnessExponent+1}}\\ &= 2\localConstantT\cdot 2^{-(j-1)\left(\tailsExponent(2\measureSmoothnessExponent+1)-1\right)} \cdot
\epsilonByNDelta^{\marginExponent+1}\cdot \epsilonByNDelta^{\mainExponentForUnboundedRiskBoundThm}.
\end{align*}
Thus, with probability at least $1-\delta$, we have
\begin{align*}
\risk\left(\est[\classifier]_{n,\delta}\right) -\risk\left(\oracle\right) & = \int_{\X} \left|\regressionFunction(x)-\frac{1}{2}\right|\cdot \one\left\lbrace \est[\classifier]_{n,\delta}(x)\neq \oracle(x)\right\rbrace d\marginalDistribution(x)\\
&\leq \int_{\goodDeltaSet} \left|\regressionFunction(x)-\frac{1}{2}\right|\cdot \one\left\lbrace \est[\classifier]_{n,\delta}(x)\neq \oracle(x)\right\rbrace d\marginalDistribution(x)+\Prob\left[\X\backslash \goodDeltaSet\right]\\
&\leq \sum_{j=0}^{\infty}\int_{\goodDeltaSetByInd[j]} \left|\regressionFunction(x)-\frac{1}{2}\right|\cdot \one\left\lbrace \est[\classifier]_{n,\delta}(x)\neq \oracle(x)\right\rbrace d\marginalDistribution(x)+\delta\leq \sum_{j=0}^{\infty}\excessErrorOnGoodDeltaSetByInd[j]+\delta\\
& \leq  \left( \marginConstant \cdot \localConstantT^{\marginExponent+1}+\sum_{j=1}^{\infty}  2\localConstantT\cdot 2^{-(j-1)\left(\tailsExponent(2\measureSmoothnessExponent+1)-1\right)} \right)\cdot \epsilonByNDelta^{\marginExponent+1}\cdot \epsilonByNDelta^{\mainExponentForUnboundedRiskBoundThm} +\delta\\
& \leq  \left( \frac{3\marginConstant \cdot \localConstantT^{\marginExponent+1}}{1-2^{1-\tailsExponent(2\measureSmoothnessExponent+1)}} \right)\cdot \epsilonByNDelta^{\marginExponent+1}\cdot \epsilonByNDelta^{\mainExponentForUnboundedRiskBoundThm} +\delta\\
& \leq C(\marginExponent,\fastLimitsExponent, \tailsExponent, \marginalDistribution) \cdot\left(1-\probFlipZeroToOne-\probFlipOneToZero\right)^{\marginExponent+1}\cdot \epsilonByNDelta^{\mainExponentForUnboundedRiskBoundThm} +\delta,
\end{align*}
where $C(\marginExponent,\fastLimitsExponent, \tailsExponent, \marginalDistribution):=\marginConstant\cdot \left(26\left(\fastLimitsConstant+2^4\cdot \doublingConstant[\marginalDistribution]\right)\right)^{\marginExponent+1}\cdot\left(1-2^{1-\tailsExponent(2\measureSmoothnessExponent+1)}\right)^{-1}$. This completes the proof of the theorem.
\end{proof}



==> Archive/inconsistency.tex <==
In this section we consider the consistency of an algorithm when trained with corrupted data. For clarity we emphasise the distinct roles of the train and test distributions in the definition of consistency. Recall that for any distribution $\Prob$ on $\X \times \{0,1\}$ and classifier $\classifier: \X \rightarrow \{0,1\}$ we let $\risk\left(\classifier;\Prob\right):= \E\left[\hat{\classifier}_n(X)\neq Y\right]$, where $\E$ denotes the expectation with respect to $\Prob$. In addition we let $\excessRisk\left(\classifier;\Prob\right)$ denote the excess risk defined by
\begin{align*}
\excessRisk\left(\classifier,\Prob\right):=\risk\left(\classifier;\Prob\right) -\inf_{\tilde{\classifier}} \left\lbrace \risk\left(\tilde{\classifier};\Prob\right)\right\rbrace,
\end{align*}
where the infimum is taken over all measureable maps $\tilde{\classifier}:\X \rightarrow \{0,1\}$. 



\begin{defn}[Consistency]\label{consistencyDefn} Let $\Prob_{\text{train}}$,$\Prob_{\text{test}}$ be probability distributions on $\X \times \{0,1\}$. We shall say that a classification algorithm $\hat{\classifier}$ is consistent with training distribution $\Prob_{\text{train}}$ and test distribution $\Prob_{\text{test}}$ if the following holds. Take $\left\lbrace (X_i,Y_i)\right\rbrace_{i\in \mathbb{N}}$ with each $(X_i,Y_i)$ sampled independently from $\Prob_{\text{train}}$. For each $n \in \N$ let $\hat{\classifier}_n$ denote the classifier obtained by applying the algorithm $\hat{\classifier}$ to the data set $\left\lbrace (X_i,\noisy[Y]_i)\right\rbrace_{i \in [n]}$. Then with probability one over $(X_i,\noisy[Y]_i) \sim \Prob_{\text{train}}$ we have 
$\lim_{n \rightarrow \infty} \excessRisk\left(\hat{\classifier}_n;\Prob_{\text{test}}\right) = 0$.
\end{defn}


A class of real-valued functions $\mathcal{F}$ is said to be a convex set if for all $f_0,f_1 \in \mathcal{F}$ and $\theta \in (0,1)$ we have $\theta \cdot f_0+(1-\theta)\cdot f_1 \in \mathcal{F}$. The class $\mathcal{F}$ is said to be a star domain if for any $f \in \mathcal{F}$ and $\theta  \in (0,1)$ we have $\theta \cdot f \in \mathcal{F}$. We let $\mathbf{1}:\X \rightarrow \R$ denote the function with $\mathbf{1}(x)=1$ for all $x \in \X$. Given a Borel probability measure $\marginalDistribution$ on $\X$ and a Borel measureable mapping $\regressionFunction:\X \rightarrow [0,1]$ we let  $\Prob_{\left(\marginalDistribution,\regressionFunction\right)}$ denote the probability distribution on $\X \times \{0,1\}$ with marginal $\marginalDistribution$ and a regression function $\regressionFunction$.

\begin{theorem}\label{inconsistencyThm} Let $\marginalDistribution$ be a Borel probability measure on $\X$ and suppose $\mathcal{F} \subset [0,1]^{\X}$ is a convex star domain consisting of Borel measureable functions with $\mathbf{1} \in \mathcal{F}$. Take probabilities $\probFlipZeroToOne, \probFlipOneToZero \in (0,1)$ with $\probFlipZeroToOne+\probFlipOneToZero<1$. Given $\regressionFunction \in \mathcal{F}$ we let $\noisy[\regressionFunction]$ be the corresponding corrupted regression function (\ref{noisyRegInTermsOfTrueRegEq}) and define
\begin{align}\label{defBayesConflictedSet}
\mathcal{A}_0(\regressionFunction):= \left\lbrace x \in \X: \left(\regressionFunction(x)-\frac{1}{2}\right)\left(\noisy[\regressionFunction](x)-\frac{1}{2}\right)<0\right\rbrace.
\end{align}
Suppose that for all $\regressionFunction \in \mathcal{F}$ the classification algorithm $\hat{\classifier}$ is consistent with both training and test distribution equal to $\Prob_{\left(\marginalDistribution,\regressionFunction\right)}$. Then for any a regression function $\regressionFunction \in \mathcal{F}$ with $\marginalDistribution\left(\mathcal{A}_0(\regressionFunction) \right)>0$ the classifier $\hat{\classifier}$ is inconsistent with training distribution $\Prob_{\left(\marginalDistribution,\noisy[\regressionFunction]\right)}$ and test distribution $\Prob_{\left(\marginalDistribution,\regressionFunction\right)}$. 
\end{theorem}
Before proving Theorem \ref{inconsistencyThm} we prove a preliminary lemma.

\begin{lemma}\label{inconsistencyLemma} Let $\marginalDistribution$ be a Borel probability measure on $\X$ and take probabilities $\probFlipZeroToOne, \probFlipOneToZero \in (0,1)$. Given $\regressionFunction:\X \rightarrow [0,1]$ and $\theta>0$ we define
\begin{align*}
\mathcal{A}_{\theta}(\regressionFunction):= \left(\left\lbrace \regressionFunction(x)\leq \frac{1}{2}-\theta  \right\rbrace\cap \left\lbrace \noisy[\regressionFunction](x)\geq \frac{1}{2}+\theta  \right\rbrace\right)\cup  \left(\left\lbrace \regressionFunction(x)\geq \frac{1}{2}+\theta  \right\rbrace\cap \left\lbrace \noisy[\regressionFunction](x)\leq \frac{1}{2}-\theta  \right\rbrace\right).
\end{align*}
Then given any classifier $\classifier: \X \rightarrow \{0,1\}$ we have $
\excessRisk\left({\classifier};\Prob_{\left(\marginalDistribution,\regressionFunction\right)}\right)+\excessRisk\left({\classifier};\Prob_{\left(\marginalDistribution,\noisy[\regressionFunction]\right)}\right) \geq \theta \cdot \marginalDistribution\left(\mathcal{A}_{\theta}(\regressionFunction)\right)$.
\end{lemma}
\begin{proof} We exploit the standard fact that for any regression function $\tilde{\regressionFunction}:\X \rightarrow [0,1]$ we have
\begin{align}\label{excessRiskEqualTo}
\excessRisk\left(\classifier;\Prob_{\left(\marginalDistribution,\tilde{\regressionFunction}\right)}\right) = \int \left| \tilde{\regressionFunction}(x)-\frac{1}{2}\right| \cdot \one \left\lbrace  \left(\tilde{\regressionFunction}(x)-\frac{1}{2}\right)\left(\classifier(x)-\frac{1}{2}\right)<0\right\rbrace d\marginalDistribution(x).
\end{align}
Now if $x \in \mathcal{A}_{\theta}(\regressionFunction)$ then $\left(\regressionFunction(x)-\frac{1}{2}\right)\left(\noisy[\regressionFunction](x)-\frac{1}{2}\right)<0$ so for all possible values $\classifier(x) \in \{0,1\}$ we have
\begin{align*}
 \one \left\lbrace  \left({\regressionFunction}(x)-\frac{1}{2}\right)\left(\classifier(x)-\frac{1}{2}\right)<0\right\rbrace +  \one \left\lbrace  \left(\noisy[\regressionFunction](x)-\frac{1}{2}\right)\left(\classifier(x)-\frac{1}{2}\right)<0\right\rbrace = 1.
\end{align*}
Moreover, if $x \in \mathcal{A}_{\theta}(\regressionFunction)$ then $\min \left\lbrace \left|{\regressionFunction}(x)-\frac{1}{2}\right|,\left|\noisy[\regressionFunction](x)-\frac{1}{2}\right| \right\rbrace\geq \theta$ and so 
\begin{align*}
\left|{\regressionFunction}(x)-\frac{1}{2}\right|\cdot \one \left\lbrace  \left({\regressionFunction}(x)-\frac{1}{2}\right)\left(\classifier(x)-\frac{1}{2}\right)<0\right\rbrace + \left|\noisy[\regressionFunction](x)-\frac{1}{2}\right|\cdot  \one \left\lbrace  \left(\noisy[\regressionFunction](x)-\frac{1}{2}\right)\left(\classifier(x)-\frac{1}{2}\right)<0\right\rbrace \geq \theta.
\end{align*}
Integrating with respect to $\marginalDistribution$ and applying (\ref{excessRiskEqualTo}) to both $\Prob_{\left(\marginalDistribution,\regressionFunction\right)}$ and $\Prob_{\left(\marginalDistribution,\noisy[\regressionFunction]\right)}$ gives the conclusion of the lemma.
\end{proof}
Theorem \ref{inconsistencyThm} now follows straightforardly.
\begin{proof}[Proof of Theorem \ref{inconsistencyThm}] Take a regression function $\regressionFunction \in \mathcal{F}$ with $\marginalDistribution\left(\mathcal{A}_0(\regressionFunction) \right)>0$. We have $\mathcal{A}_0(\regressionFunction) = \bigcup_{\theta>0}\mathcal{A}_{\theta}(\regressionFunction)$ and hence
\begin{align*}
\lim_{\theta \rightarrow 0}\left\lbrace \marginalDistribution\left( \mathcal{A}_{\theta}(\regressionFunction)\right) \right\rbrace = \marginalDistribution\left(\mathcal{A}_0(\regressionFunction) \right)>0.
\end{align*}
Thus, we may choose some $\theta>0$ with $\marginalDistribution\left( \mathcal{A}_{\theta}(\regressionFunction)\right) >0$. By Lemma \ref{inconsistencyLemma} we have
\begin{align}\label{ineqApplyingInconsistencyLemma}
\excessRisk\left({\classifier};\Prob_{\left(\marginalDistribution,\regressionFunction\right)}\right)+\excessRisk\left({\classifier};\Prob_{\left(\marginalDistribution,\noisy[\regressionFunction]\right)}\right) \geq \theta \cdot \marginalDistribution\left(\mathcal{A}_{\theta}(\regressionFunction)\right)>0.
\end{align}
Since $\regressionFunction \in \mathcal{F}$ and  $\mathcal{F} \subset [0,1]^{\X}$ is a convex star domain consisting of Borel measureable functions with $\mathbf{1} \in \mathcal{F}$ we also have $\noisy[\regressionFunction]=\left(1-\probFlipZeroToOne-\probFlipOneToZero\right) \cdot \regressionFunction(x)+\probFlipZeroToOne \in \mathcal{F}$. Hence, $\hat{\classifier}$ is consistent on with train and test disribution equal to $\Prob_{\left(\marginalDistribution,\noisy[\regressionFunction]\right)}$. Thus, $\lim_{n \rightarrow \infty}\excessRisk\left(\hat{\classifier}_n;\Prob_{\left(\marginalDistribution,\noisy[\regressionFunction]\right)}\right) = 0$. By applying (\ref{ineqApplyingInconsistencyLemma}) it follows that $\limsup_{n \rightarrow \infty}\excessRisk\left(\hat{\classifier}_n;\Prob_{\left(\marginalDistribution,{\regressionFunction}\right)}\right)$. Hence, $\hat{\classifier}$ is inconsistent when trained with train distribution  $\Prob_{\left(\marginalDistribution,\noisy[\regressionFunction]\right)}$ and test distribution  $\Prob_{\left(\marginalDistribution,{\regressionFunction}\right)}$.
\end{proof}

\begin{corollary} Let $\hat{\classifier}$ denote the $k$-nearest neighbour with $k_n/n \rightarrow 0$ and $k_n/n \rightarrow \infty$, where $k_n$ is the number of neighbours applied to a data set of size $n$. Suppose we have a regression function $\regressionFunction:\X \rightarrow [0,1]$ such that $\marginalDistribution\left(\mathcal{A}_0(\regressionFunction) \right)>0$ and for $\marginalDistribution$ almost every $x \in \X$,
\begin{align*}
\lim_{r\rightarrow 0}\frac{1}{\marginalDistribution\left(B_r(x)\right)} \int_{B(x,r)}\regressionFunction\hspace{1mm} d\marginalDistribution = \regressionFunction(x).
\end{align*}
Then the $k$-nearest neighbour classifier is inconsistent with training distribution $\Prob_{\left(\marginalDistribution,\noisy[\regressionFunction]\right)}$ and test distribution $\Prob_{\left(\marginalDistribution,\regressionFunction\right)}$.
\end{corollary}

==> Archive/introduction.tex <==
%\DeclareDocumentCommand\foo{ m O{x} m }{ A #1 A #2 A #3 A }

Traditionally, the statistical analysis of supervised learning assumes a perfectly labelled training set. However, there is an increasing realisation that label noise is a common occurrence. Real-world data has been estimated to contain around 5\% encoding errors already 20 years ago \cite{Orr,Redman}, and for massive data sets, perfectly accurate labels are very costly, if not impossible, to produce. 
In turn, %croudsourcing allows one to 
imperfect labels can often be cheaply obtained %via services such as the Amazon Mechanical Turk, which could be made good use of. C
and consequently, an increasing body of literature concerns the study of classification with label noise. % -- reviews many be found e.g. in \cite{Frenay1,Frenay2}.

In this work we consider asymmetric random label noise with unknown class-conditional noise proportions: Instead of clean labels we can only observe corrupted labels that have been randomly flipped in some proportion that differs in each class. This type of noise is known to deteriorate the predictive performance of learning algorithms in general, and as we shall point out, even consistency guarantees may be lost. 

The practical relevance of class-conditional asymmetric label noise is widely evidenced in the literature, see for instance the recent works of \cite{blanchard2016,natarajan2018} and references therein. Class conditional random label noise represents a noise model that is both realistic and amenable to analysis -- reasons for which it was subject of several theoretical studies that aim to better understand the impact of label noise. However, most of these assume that the noise proportions are known. In particular, the recent study in \cite{natarajan2018} works under the assumption of some approximate knowledge of the noise proportions.

The requirement to know the noise proportions beforehand is a limiting factor both in practice and in terms of theoretical understanding. In many situations such knowledge is not available. 
As a concrete example, in positive unlabelled (PU) learning \cite{ElkanNoto} one may regard unlabelled data as a class of negative examples contaminated with positives in an unknown proportion. The work of \cite{blanchard2016} discusses further application areas where the noise proportions are unknown, including an application in high energy Physics. 
They also establish necessary and sufficient conditions for the identifyability of the clean class-conditional distributions and the noise proportions, which consist of the requirement that the majority of the observed labels are clean, and an irreducibility condition. The latter condition was shown \cite{menon2015learning} to be equivalent to a condition on the extrema of the true regression function.

In \cite{blanchard2016} it was also shown that the identifyability conditions are insufficient to obtain finite sample convergence rates. Under additional conditions external to the classification task, \cite{scott2015rate} obtained the parametric rate, i.e. of order $n^{-1/2}$ where $n$ is the sample size. To the best of our knowledge it is unknown whether better rates are possible.

A faster rate would mean that less data is required for the same classification accuracy. The study of convergence rates is therefore a central topic of study in statistical machine learning. We are unaware of fast rates in the presence of label noise, with the exception of recent work of \cite{cannings2018}, in which the authors consider a different types of noise, and their goal is to identify extra conditions under which the existing traditional classifiers would retain their guarantees in the presence of label noise.

This paper is motivated by two fundamental questions: 
1) Assuming conditions that ensure minimax optimal fast rates in the noise free setting, would the label noise identifyability conditions suffice to obtain the same minimax optimal fast rates?
2) What characteristics of the true underlying data distribution influence the rate, and how does the rate behave as a function of these characteristics? 

Our high level strategy is generic for the type of label noise considered, although we focus on nearest neighbour based plug-in methods and develop detailed analysis in this setting.
The specific contributions of of this paper are the following:
\begin{itemize}
    \item We show that a Bayes consistent method becomes inconsistent when applied to data with unknown asymmetric label noise. This is in contrast with claims about the surprising robustness of high capacity models to class-dependent label noise when given sufficient amounts of data, (e.g. summarised in the introductory section of \cite{MenonMLJ2018} from references therein) %\cite{patrini2017}, 
    which (explicitly or tacitly) assume either that the label noise proportions are known, or that the label noise is is symmetric.
    \item We show that it is possible to attain nearly minimax optimal rates despite the presence of unknown asymmetric label noise, under the measure smoothness condition introduced in recent analyses of kNN in the noise-free setting \cite{chaudhuri2014rates} (termed also as "modified Lipschitz" condition in \cite{doring2018}) with the only addition of the noise identifyability conditions \cite{blanchard2016}, and fast rates are attained whenever Tysbakov's noise condition holds. 
    \item We introduce a new local measure smoothness condition that generalises the framework of \cite{gadat2016}.
    and allows consideration of general unbounded input domains provided that an assumption of tail decay is made on the marginal distribution. Our analysis in this setting reveals that the rate depends on the speed at which the class posterior (or regression function) approaches its extrema relative to the tail decay of the marginal distribution, and it exhibits a threshold behaviour: 
    \begin{itemize}
        \item The noise-free nearly minimax optimal rate of this setting \cite{gadat2016} is again attainable if the regression function approaches its extrema faster than a threshold. 
        \item Otherwise the rate is slower than in the noise-free case. [? can we say this?: However, we also show that this slower rate is minimax optimal in the presence of label-noise. Therefore we identified a characteristic of the underlying distribution responsible for the statistical difficulty of learning with label noise.
        ]
\end{itemize}
\end{itemize}

Our analysis applies in general metric spaces and does not require the marginal distribution to have a density.

==> Archive/kNNForLabelNoiseGeneralBounds.tex <==
The $k$-nearest neighbour method for asymmetric label noise is the special case of the plug-in method (Algorithm \ref{classificationBasedOnCorruptedRegressionFunctionAlgo}) in which we use the $k$-nearest neighbour method to estimate the corrupted regression function and use empirical minima and maxima to estimate the noise probabilities (Algorithm \ref{simpleKNNBasedOnCorruptedRegressionFunctionAlgo}). REF??? GAO paper???? The first stage in analysing Algorithm \ref{simpleKNNBasedOnCorruptedRegressionFunctionAlgo} is to understand how well the empirical maxima estimate the true maximum of the function.


\begin{algorithm}[htbp]
%\floatconts
%{alg:KNNInd}
 {\caption{The $k$-NN method with label noise\label{simpleKNNBasedOnCorruptedRegressionFunctionAlgo}}}
{ 
 \begin{enumerate}
     \item Construct the $k$-NN estimate of the corrupted regression function $\left(\noisy[{\est[\regressionFunction]}]\right)_{n,k}$ based on $\noisy[\sample]$;
     \item Compute $\estProbFlipZeroToOne=\min_{i \in [n]}\left\lbrace \left(\noisy[{\est[\regressionFunction]}]\right)_{n,k}(X_i)\right\rbrace$ and $\estProbFlipOneToZero=1-\max_{i \in [n]}\left\lbrace \left(\noisy[{\est[\regressionFunction]}]\right)_{n,k}(X_i)\right\rbrace$;
     \item Let $\KNNClassifier(x):= \one\left\lbrace \left(\noisy[{\est[\regressionFunction]}]\right)_{n,k}(x) \geq 1/2 \cdot \left(1+\estProbFlipZeroToOne-\estProbFlipOneToZero\right) \right\rbrace$.
     \end{enumerate}
 }
\end{algorithm}

\subsection{Estimating the maximum of a function with $k$ nearest neighbours}

In this section we present a general result which describes bounds the performance of the empirical maximum of the $k$-NN estimate of a function as an estimator of its supremum. As in Section \ref{KNNFuncEstSec}, we shall assume we have access to a sample $\sample_f = \left\lbrace \left(X_i,Z_i\right)\right\rbrace_{i \in [n]}$ with $(X_i,Z_i) \sim \Prob$ generated i.i.d. where $\Prob$ is an unknown distribution on $\X \times [0,1]$ with $f(x)= \E\left[Z|X=x\right]$. Our aim is to estimate $M(f):=\sup_{x \in \suppMarginalDistribution}\left\lbrace f(x) \right\rbrace$ based on $\sample_f$. We let $\KNNMaxEstimate$ denote the empirical maximum of the $k$-NN estimate
$\KNNMaxEstimate:= \max_{i \in [n]}\left\lbrace \KNNest(X_i) \right\rbrace$. In addition, for each $p \in (0,1)$ we define
\begin{align*}
\PMax{f}{p}:=\sup_{x_0 \in \X}\left\lbrace \left(f^-_p\right)^-_p(x_0)\right\rbrace =\sup_{x_0 \in \X}\left\lbrace \inf_{x_1 \in \X}\left\lbrace \inf_{x_2 \in \X}\left\lbrace f(x_2): \dist(x_1,x_2)\leq \PRadius{p}{x_1} \right\rbrace:  \dist(x_0,x_1)\leq \PRadius{p}{x_0}\right\rbrace\right\rbrace.
\end{align*}
?????We also let $\PMin{f}{p}:=\inf_{x_0 \in \X}\left\lbrace \left(f^+_p\right)^+_p(x_0)\right\rbrace= 1-\PMax{1-f}{p}$.

\begin{theorem}[k-NN maximum bound]\label{KNNMaxBoundThm} Let $f:\X \rightarrow [0,1]$ be a Borel measurable function. Take $n \in \N$, $\delta \in \left(0,1\right)$ and $k \in \{\lceil 8\log((8n)/\delta)+1\rceil,\cdots, \lfloor n/2 \rfloor\}$ and let $p=(2k)/n$. It follows that with probability at least $1-\delta$ over $\sample_f$
\begin{align}
\PMax{f}{p}-\sqrt{\frac{\log((8n)/\delta)}{2k}} \leq \KNNMaxEstimate \leq M(f)+\sqrt{\frac{\log((8n)/\delta)}{2k}}.
\end{align}
\end{theorem}
\begin{proof}
Note that it suffices to show that for each $l \in \N$ the following holds with probability at least $1-\delta$ over $\sample_f$,
\begin{align}\label{keyClaimInPfOfKNNMaxBoundThm}
\PMax{f}{p}-\frac{1}{l}-\sqrt{\frac{\log((8n)/\delta)}{2k}} \leq \KNNMaxEstimate \leq M(f)+\sqrt{\frac{\log((8n)/\delta)}{2k}}.
\end{align}
We can then apply continuity from above to the interesection of all events where (\ref{keyClaimInPfOfKNNMaxBoundThm}) hold for $l \in \N$. Hence, we fix $l \in \N$, choose $x_0 \in \X$ so that $\left(f^-_{p}\right)^-_{p}(x_0)>\PMax{f}{p}-1/l$ and proceed to prove that (\ref{keyClaimInPfOfKNNMaxBoundThm}) holds with high probability. Now take $B_0:= \left\lbrace x \in \X: \dist\left(x,x_0\right)\leq r_{p}(x_0)\right\rbrace = \bigcap_{r>r_{p}(x_0)}B_r(x_0)$. It follows that $\marginalDistribution\left(B_0\right)\geq {p}$. Hence, we have
\begin{align*}
\Prob_{\Xsample}\left[ \dist\left(X_{\tau_{n,1}(x_0)},x_0\right)>r_{p}(x_0) \right]& = \Prob_{\Xsample}\left[ \left\lbrace X_i\right\rbrace_{i \in [n]} \cap B_0 = \emptyset \right] \leq \left(1-\frac{2k}{n}\right)^n \leq \exp(-2k) \leq \delta/2.
\end{align*}
Thus, with probability at least $1-\delta/2$ over $\sample_f$ we have
\begin{align}\label{PfOfMaxKNNMaxPointHasClose1NN}
\dist\left(X_{\tau_{n,1}(x_0)},x_0\right)\leq r_{p}(x_0).
\end{align}
Moreover, by Theorem \ref{KNNPointwiseBoundFixedKThm} the following holds  with probability at least $1-\delta/2$ simultaneously for all $i \in [n]$,
\begin{align}\label{unionOverDataBoundInPfOfMaxKNNBound}
\lowerPRadiusBound{f}{p}{X_i}-\sqrt{\frac{\log((8n)/\delta)}{2k}} \leq \KNNest[f](X_i) \leq \upperPRadiusBound{f}{p}{X_i}+\sqrt{\frac{\log((8n)/\delta)}{2k}}.
\end{align}
By the union bound (\ref{PfOfMaxKNNMaxPointHasClose1NN}) and (\ref{unionOverDataBoundInPfOfMaxKNNBound}) hold simultanously with probability at least  $1-\delta$ over $\sample_f$. Hence, it suffices to assume (\ref{PfOfMaxKNNMaxPointHasClose1NN}) and (\ref{unionOverDataBoundInPfOfMaxKNNBound}) and deduce (\ref{keyClaimInPfOfKNNMaxBoundThm}). The upper bound follows straightforwardly from (\ref{unionOverDataBoundInPfOfMaxKNNBound}). Indeed, for each $i \in [n]$ we have $\upperPRadiusBound{f}{p}{X_i}= \sup_{\tilde{x} \in \X}\left\lbrace f(\tilde{x}): \dist(\tilde{x},X_i)\leq \PRadius{p}{X_i}\right\rbrace \leq M(f)$. By the upper bound in (\ref{keyClaimInPfOfKNNMaxBoundThm}) we infer that $\KNNMaxEstimate \leq M(f)+\sqrt{{\log((8n)/\delta)}/{(2k)}}$. On the other hand, it follows from (\ref{PfOfMaxKNNMaxPointHasClose1NN}) that for any function $g:\X\rightarrow [0,1]$ we have $g(X_{\tau_{n,1}(x_0)}) \geq g^-_{p}(x_0)$. In particular, $f^-_{p}(X_{\tau_{n,1}(x_0)}) \geq \left(f^-_{p}\right)^-_{p}(x_0)$. By combining with the lower bound in (\ref{unionOverDataBoundInPfOfMaxKNNBound}) we obtain
\begin{align*}
\KNNMaxEstimate & \geq \KNNest(X_{\tau_{n,1}(x_0)}) \geq 
\lowerPRadiusBound{f}{p}{X_{\tau_{n,1}(x_0)}}-\sqrt{\frac{\log((8n)/\delta)}{2k}} \\& \geq  \left(f^-_{p}\right)^-_{p}(x_0) -\sqrt{\frac{\log((8n)/\delta)}{2k}} \\ &> \PMax{f}{p}-\frac{1}{l}-\sqrt{\frac{\log((8n)/\delta)}{2k}}.
\end{align*}
Thus, (\ref{keyClaimInPfOfKNNMaxBoundThm}) holds with probability at least  $1-\delta$ over $\sample_f$. This completes the proof of the theorem.
\end{proof}


\subsection{Bounding the mis-classification rate for the $k$-NN method with asymmetric label noise}

We shall now use Theorem \ref{KNNMaxBoundThm} to give a high probability upper bound on the mis-classification rate for Algorithm \ref{simpleKNNBasedOnCorruptedRegressionFunctionAlgo}. We shall use the following lemma.

\begin{lemma}\label{elementaryRatioLemma} Suppose that $\estProbFlipZeroToOne, \estProbFlipOneToZero \in \left[0,1\right)$ with $\estProbFlipZeroToOne+\estProbFlipOneToZero<1$. Let $\noisy[{\est[\regressionFunction]}]:\X \rightarrow [0,1]$ be an estimate of $\noisyRegressionFunction$ and define $\est[\regressionFunction] :\X \rightarrow [0,1]$ by $\est[\regressionFunction](x):= \left(\noisy[{\est[\regressionFunction]}](x)-\estProbFlipZeroToOne\right)/\left(1-\estProbFlipZeroToOne-\estProbFlipOneToZero\right)$. Suppose that $\probFlipZeroToOne+\probFlipOneToZero<1$ and $\max\left\lbrace\left| \estProbFlipZeroToOne-\probFlipZeroToOne \right|, \left| \estProbFlipOneToZero-\probFlipOneToZero \right| \right\rbrace  \leq \left(1-\probFlipZeroToOne-\probFlipOneToZero\right)/4$. Then for all $x \in \X$ we have
\begin{align*}
\left| \est[\regressionFunction](x)-\regressionFunction(x)\right| \leq\frac{6}{ \left(1-\probFlipZeroToOne-\probFlipOneToZero\right)^{2}} \cdot \max\left\lbrace \left| \estNoisyRegressionFunction(x) - \noisyRegressionFunction(x)\right|, \left| \estProbFlipZeroToOne-\probFlipZeroToOne \right|, \left| \estProbFlipOneToZero-\probFlipOneToZero \right| \right\rbrace.
\end{align*}
\end{lemma}
\begin{proof}
Follows straightforwardly from (\ref{noisyRegInTermsOfTrueRegEq})).
\end{proof}

For each $p \in \left(0,1\right)$ and $\Delta>0$ we define
\begin{align*}
\positiveRegion&:=\left\lbrace x\in \suppMarginalDistribution:\forall \tilde{x} \in \suppMarginalDistribution \text{ with }\dist\left(\tilde{x},x\right) \leq r_p(x)\text{ we have }\regressionFunction(\tilde{x}) >\frac{1}{2}+\Delta \right\rbrace\\
\negativeRegion&:=\left\lbrace x\in \suppMarginalDistribution:\forall \tilde{x} \in \suppMarginalDistribution \text{ with }\dist\left(\tilde{x},x\right) \leq r_p(x)\text{ we have }\regressionFunction(\tilde{x}) <\frac{1}{2}-\Delta \right\rbrace,
\end{align*}
and let $\boundary:=\X\backslash \left(\positiveRegion \cup \negativeRegion\right)$. Recall that $\oracle(x)= \one\left\lbrace \regressionFunction(x) \geq \frac{1}{2}\right\rbrace$.




\begin{theorem}[General mis-classification bound]\label{KNNMisclassificationGeneralBoundThm} Take $n \in \N$, $\delta \in \left(0,1\right)$ and $k \in \{\lceil 16\log((6n)/\delta)+1\rceil,\cdots, \lfloor n/2 \rfloor\}$, let $p=(2k)/n$ and take
\begin{align}\label{deltaDefInKNNMisclassificationGeneralBoundThm}
\Delta =  \frac{6}{ \left(1-\probFlipZeroToOne-\probFlipOneToZero\right)^{2}} \cdot \left( \max\left\lbrace 1-M_p(\regressionFunction),1-M_p(1-\regressionFunction)\right\rbrace+\sqrt{\frac{\log((6n)/\delta)}{k}}\right).    
\end{align}
It follows that with probability at least $1-\delta$ over $\sample_f$ we have
\begin{align*}
\marginalDistribution\left( \left\lbrace x \in \X: \KNNClassifier(x) \neq \oracle(x) \right\rbrace\right) \leq \marginalDistribution\left(\boundary\right)+\delta.
\end{align*}

\end{theorem}






































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































==> Archive/kNearestNeighbourRegression.tex <==
In this section we consider supervised $k$-nearest neighbour regression. Whilst we are motivated by the estimation of $\noisy[\regressionFunction]$ we shall frame our results in a more general fashion for clarity. Suppose we have a distribution $\Prob$ on $\X \times [0,1]$ and let $f:\X\rightarrow [0,1]$ be the function $f(x):= \E\left[Z|X=x\right]$. Our goal is to estimate $f$ based on a sample $\sample_f = \left\lbrace \left(X_i,Z_i\right)\right\rbrace_{i \in [n]}$ with $(X_i,Z_i) \sim \Prob$ generated i.i.d. Given $x \in \X$ we define let $\left\lbrace \tau_{n,q}(x)\right\rbrace_{q \in [n]}$ be a data-dependent enumeration of $[n]$ such that for each $q \in [n-1]$, $\rho\left(x,X_{\tau_{n,q}(x)}\right) \leq \rho\left(x,X_{\tau_{n,q+1}(x)}\right)$. We define the $k$-nearest neighbour estimate $\KNNest[f]: \X \rightarrow [0,1]$ of $f$ by 
\begin{align*}
\KNNest[f](x):=\frac{1}{k} \cdot \sum_{q \in [k]}Z_{\tau_{n,q}(x)}.
\end{align*}
Given a point $x \in \X$ and $r>0$ we define $\openBall{r}{x}=\left\lbrace \tilde{x} \in \X: \dist(x,\tilde{x})<r\right\rbrace$. For each $x \in \X$ and $p \in \left(0,1\right)$ we let $\PRadius{p}{x}:=\inf\left\lbrace r>0:\marginalDistribution\left(\openBall{r}{x}\right) \geq p\right\rbrace$ and define
\begin{align*}
\upperPRadiusBound{f}{p}{x}:=\sup_{\tilde{x} \in \X}\left\lbrace f(\tilde{x}): \dist(\tilde{x},x)\leq \PRadius{p}{x}\right\rbrace.
\end{align*}
We define $\lowerPRadiusBound{f}{p}{x}$ similarly, but with the infimum in place of the supremum. We shall use $f^+_p$ and $f^-_p$ to give a general bounds on the $k$-nearest neighbour estimate $\KNNest[f]$.


\begin{theorem}[k-nearest neighbour bound]\label{KNNPointwiseBoundFixedKThm} Let $f:\X \rightarrow [0,1]$ be a Borel measurable function. Given any $x \in \X$, $n \in \N$, $\delta \in \left(0,1\right)$ and $k \in \{\lceil 8\log(4/\delta)\rceil,\cdots, \lfloor n/2 \rfloor\}$, the following holds with probability at least $1-\delta$ over $\sample_f$,
\begin{align}\label{deterministicBoundInPfOfKNNPointwiseBoundFixedKThm}
\lowerPRadiusBound{f}{(2k)/n}{x}-\sqrt{\frac{\log(4/\delta)}{2k}} \leq \KNNest[f](x) \leq \upperPRadiusBound{f}{(2k)/n}{x}+\sqrt{\frac{\log(4/\delta)}{2k}}.
\end{align}
Moreover, whenever $k\geq 8\log((4n)/\delta)+1$ the following bound holds simultaneously for all $j \in [n]$ with probability at least $1-\delta$ over $\sample_f$,
\begin{align}\label{unionOverDataBoundInPfOfKNNPointwiseBoundFixedKThm}
\lowerPRadiusBound{f}{(2k)/n}{X_j}-\sqrt{\frac{\log((4n)/\delta)}{2k}} \leq \KNNest[f](X_j) \leq \upperPRadiusBound{f}{(2k)/n}{X_j}+\sqrt{\frac{\log((4n)/\delta)}{2k}}.
\end{align}
\end{theorem}
Theorem \ref{KNNPointwiseBoundFixedKThm} gives point-wise bounds on the k nearest neighbour regression estimator. The proof relies upon two lemmas. Let $\Xsample = \left\lbrace X_i\right\rbrace_{i \in [n]}$ and $\Zsample=\left\lbrace Z_i\right\rbrace_{i \in [n]}$ and define $\conditionalExpectKNNest[f](x)=\E_{\Zsample|\Xsample}\left[\KNNest[f](x)\right] =\frac{1}{k} \cdot \sum_{q \in [k]}f\left(X_{\tau_{n,q}(x)}\right)$.

 \begin{restatable}{lemma}{knnEstIsCloseToItsXConditionalExpectationLemma}\label{knnEstIsCloseToItsXConditionalExpectationLemma} With $x,n,k$ as in Theorem \ref{KNNPointwiseBoundFixedKThm} for each $\xi>0$ we have
$\Prob_{\Zsample|\Xsample}\left[ \KNNest[f](x)\leq \conditionalExpectKNNest[f](x)+\xi \right] \leq \exp\left(-2k \cdot \xi^2\right)$.
 \end{restatable}
\begin{proof}Follows from Hoeffding's inequality for bounded random variables \cite{boucheron2013concentration}.
\end{proof}


The second lemma is due to Chaudhuri and Dasgupta \cite{chaudhuri2014rates}.

\begin{restatable}[Chaudhuri \& Dasgupta]{lemma}{closeNeighboursFixedPointLemma}\label{closeNeighboursFixedPointLemma} Take $x \in \X$, $k \in [n]$ and $p\in [k/n,1]$. Then
\begin{align*}
\Prob_{\sample}\left[ \rho\left(x,X_{\tau_{n,k}(x)}\right) > r_p(x)\right] \leq \exp\left(-\frac{k}{2}\cdot\left(1-\frac{k}{np}\right)^2\right).
 \end{align*}
\end{restatable}
\begin{proof} Follows straightforwardly from the multiplicative Chernoff bound.
\end{proof}
We now prove Theorem \ref{KNNPointwiseBoundFixedKThm} by combining lemmas \ref{knnEstIsCloseToItsXConditionalExpectationLemma} and \ref{knnEstIsCloseToItsXConditionalExpectationLemma}.

\begin{proof}[Proof of Theorem \ref{KNNPointwiseBoundFixedKThm}] First note that for both bounds (\ref{deterministicBoundInPfOfKNNPointwiseBoundFixedKThm} \& \ref{unionOverDataBoundInPfOfKNNPointwiseBoundFixedKThm}) in Theorem \ref{KNNPointwiseBoundFixedKThm} it suffices to prove that the upper bounds hold with probability at least $1-\delta/2$. We can then deduce the lower bound by applying the upper bound to the function $1-f$ and then combine the upper and lower bounds via the union bound.

We start with the first upper bound (\ref{deterministicBoundInPfOfKNNPointwiseBoundFixedKThm}). Take $p=2k/n$. By Lemma \ref{closeNeighboursFixedPointLemma} combined with $k\geq 8\log(4/\delta)$ we have $\rho\left(x,X_{\tau_{n,k}(x)}\right) \leq r_p(x)$ with probability at least $1-\delta/4$. Note that this implies $\rho\left(x,X_{\tau_{n,q}(x)}\right) \leq r_p(x)$ for all $q \in [k]$ and hence $ \conditionalExpectKNNest[f](x)\leq \upperPRadiusBound{f}{p}{x}$. Moreover, by Lemma \ref{knnEstIsCloseToItsXConditionalExpectationLemma} we also have $\KNNest[f](x)\leq \conditionalExpectKNNest[f](x)+\sqrt{\log(4/\delta)/(2k)}$ with probability at least $1-\delta/4$. Hence, with probability at least $1-\delta/2$, the upper bound in (\ref{deterministicBoundInPfOfKNNPointwiseBoundFixedKThm}) holds. 

We now turn to the second bound (\ref{unionOverDataBoundInPfOfKNNPointwiseBoundFixedKThm}). First consider the random variable $X_n$. By applying Lemma \ref{closeNeighboursFixedPointLemma} to the reduced data set $\sample_f^{(n-1)} = \left\lbrace \left(X_i,Z_i\right)\right\rbrace_{i \in [n-1]}$ and noting that $k \geq 8 \log((4n)/\delta)+1$ we see that with probability at least $1-\delta/(4n)$ we have 
\begin{align*}
\rho\left(X_n,X_{\tau_{n,k}(X_n)}\right) =\rho\left(X_n,X_{\tau_{n-1,k-1}(X_n)}\right) \leq r_{(2(k-1))/(n-1)}(X_n)\leq r_{(2k)/n}(X_n).    
\end{align*}
 Moreover, by Lemma \ref{knnEstIsCloseToItsXConditionalExpectationLemma} we also have $\KNNest[f](X_n)\leq \conditionalExpectKNNest[f](X_n)+\sqrt{\log((4n)/\delta)/(2k)}$ with probability at least $1-\delta/(4n)$.
Hence, with probability at least $1-\delta/(2n)$ over $\sample_f$ we have
\begin{align*}
\KNNest[f](X_n) \leq \upperPRadiusBound{f}{(2k)/n}{X_n}+\sqrt{\frac{\log((4n)/\delta)}{2k}}.
\end{align*}
By symmetry the above high probability bound holds for each $j \in [n]$ with $X_j$ in place of $X_n$. Thus, taking the union bound over all $j \in [n]$ we deduce the upper bound in \ref{unionOverDataBoundInPfOfKNNPointwiseBoundFixedKThm} with probability at least $1-\delta/2$ over $\sample_f$.
\end{proof}


%https://page.mi.fu-berlin.de/mulzer/notes/misc/chernoff.pdf

==> Archive/lowerBoundProofOld.tex <==
\subsection{A lower bound for unknown label noise}\label{LBForUnknownLabelNoiseAppendix}

The goal of this section is to prove Proposition \ref{lowerBoundWithUnknownNoise} which corresponds to the difficulty of estimating the noise probabilities and the resultant effect upon classification risk.

\begin{prop}\label{lowerBoundWithUnknownNoise} 
Take $\Gamma = (\maxAggregateFlippingProbability,(\marginExponent,\marginConstant),(\holderExponent,\holderConstant),  (\dimensionExponent,\dimensionRadius),(\tailsExponent,\tailsConstant), ( \fastLimitsExponent, \fastLimitsThreshold, \fastLimitsConstant) )$ consisting of exponents $\marginExponent \in [0,\infty)$, $\holderExponent \in (0,1]$, $\dimensionExponent \in [\marginExponent\holderExponent,\infty)$, $\tailsExponent \in (0,1]$, $\fastLimitsExponent \in (0, \infty)$ and constants $\maxAggregateFlippingProbability \in (0,1)$, $\marginConstant \geq 4^{\marginExponent}$, $\marginConstant$, $\holderConstant$, $\tailsConstant$, $\fastLimitsConstant \geq 1$ and $\tailsThreshold \in (0,1/24)$, $\fastLimitsThreshold \in (0,1/3)$. There exists a constant $c_0$, depending solely upon $\Gamma$, such that for any $n \in \N$ and any classifier $\classifier$ which is measurable with respect to the corrupted sample $\noisySample$, there exists a distribution $\Prob \in \distributionClass(\Gamma)$ such that 
\begin{align*}
\ExpectationOverNoisySamples\left[ \risk\left(\classifier\right) \right] -  \risk\left(\oracle\right) \geq c_0 \cdot n^{-\frac{\fastLimitsExponent \holderExponent(\marginExponent+1)}{\fastLimitsExponent(2\holderExponent+\dimensionExponent)+\holderExponent}}.
\end{align*}
\end{prop}


\newcommand{\volA}{u}
\newcommand{\densityA}{w}
\newcommand{\volC}{v}

To prove Proposition \ref{lowerBoundWithUnknownNoise} we will show that there exists a pair of distributions $\Prob^0$ and $\Prob^1$ such that whilst the corrupted regression functions ($\noisy[\regressionFunction]^0$ and $\noisy[\regressionFunction]^1$) closely resemble one another, the true regression functions ($\regressionFunction^0$ and $\regressionFunction^1$) are substantially different. Thus, whilst it is difficult to distinguish $\Prob^0$ and $\Prob^1$ based upon the corrupted sample $\noisySample$, failing to do so results in substantial misclassification error. Figure \ref{figForLowerBound} in Section \ref{mainLBSec} illustrates the construction. To formalise this idea we require the following variant of Fano's lemma due to \cite{birge2001new}.

\begin{lem}[Birg\'{e}]\label{birgesVersionOfFanosLemma} Given a finite family $\mathcal{S}$ consisting of probability measures on a measureable space $\left(\mathcal{Z},\Sigma\right)$ and a random variable $Z$ with an unknown distribution in the family, then we have
\begin{align*}
\inf_{\hat{T}}\left\lbrace \sup_{{\Prob}_Z\in \mathcal{S}}\left\lbrace \Prob_Z\left[\hat{T}(Z) \neq \Prob_Z\right]\right\rbrace\right\rbrace \geq \min\left\lbrace 0.36,1- \inf_{\Prob_Z \in \mathcal{S}}\left\lbrace \sum_{\tilde{\Prob}_Z \in \mathcal{S}} \frac{\kullbackLeiblerDivergence\left(\Prob_Z,\tilde{\Prob}_Z\right)}{\left|\mathcal{S}\right|\log\left|\mathcal{S}\right|}  \right\rbrace\right\rbrace,
\end{align*}
where the infimum is taken over all measureable (possibly randomised) estimators $\hat{T}:\mathcal{Z}\rightarrow \mathcal{S}$.
\end{lem}


\newcommand{\twoMeasuresUnknownNoiseDistIndex}{\iota}

We apply Lemma \ref{birgesVersionOfFanosLemma} as follows: Given an integer $n \in \N$ and a quintuple $\left(\Delta,r, \volA, \volC,\densityA \right) \in (0,1/6)^5$ (to be selected in terms of $n$ later) we shall construct a measureable space with a pair of distributions. First we construct a metric space by letting $\X = \{a,b,c,d\}$ and choosing $\dist$ such that 
\begin{align*}
\dist(x_0,x_1)& =  r &\text{ if }&x_0,x_1 \in \{a,b\}\text{ and }x_0\neq x_1\\
\dist(x_0,x_1)& \geq 1 &\text{ if }&x_0 \notin \{a,b\}\text{ or }x_1 \notin\{a,b\} \text{ and }x_0\neq x_1\\
\dist(x_0,x_1)&=0 &\text{ if }&x_0 = x_1.
\end{align*}
Note that there are metric spaces $(\X,\dist)$ of this form embedded isometrically in any Euclidean space $(\R^D,\|\cdot\|_2)$. We shall define a pair of probability distributions $\Prob^0,\Prob^1$ over random triples $(X,Y,\tilde{Y}) \in \X\times \Y^2$ as follows. First we define a Borel probability measure $\marginalDistribution$ on $\X$ by $\marginalDistribution(\{a\}) = \volA$, $\marginalDistribution(\{b\}) = 1/3$, $\marginalDistribution(\{c\}) = \volC$ and $\marginalDistribution(\{d\}) = 2/3-\volA-\volC$. Second, we define a pair of regression functions $\regressionFunction^0,\regressionFunction^1:\X\rightarrow [0,1]$ on $\X$ as follows by 
\begin{align*}
\regressionFunction^0(a)&=1,&
\hspace{1cm}\regressionFunction^0(b)&=1-\Delta,& \hspace{1cm}\regressionFunction^0(c)&=\frac{1-\Delta}{2-\Delta}&
\hspace{1cm}\regressionFunction^0(d)&=0\\
\regressionFunction^1(a)&=1,&
\regressionFunction^1(b)&=1,&
\regressionFunction^1(c)&=\frac{1}{2-\Delta}&
\regressionFunction^1(d)&=0.
\end{align*}
Third, we define probabilities $\probFlipFrom[j]^{\twoMeasuresUnknownNoiseDistIndex}\in (0,1)$ for $\{\twoMeasuresUnknownNoiseDistIndex,j\} \in \{0,1\}$ by taking $\probFlipZeroToOne^0=\probFlipOneToZero^0=0$, $\probFlipOneToZero^0=1/4$ and $\probFlipOneToZero^1=(1+3\Delta)/4$. We then put these pieces together by taking, for each ${\twoMeasuresUnknownNoiseDistIndex}\in \{0,1\}$, $\Prob^{\twoMeasuresUnknownNoiseDistIndex}$ to be the unique distribution on $(X,Y,\tilde{Y}) \in \X\times \Y^2$ with (a) marginal distribution $\marginalDistribution$, (b) regression function $\regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(x)=\Prob^{\twoMeasuresUnknownNoiseDistIndex}[Y=1|X=x]$ and (c) label noise probabilities $\probFlipFrom[j]^{\twoMeasuresUnknownNoiseDistIndex}$. In addition, we define $\densityFunction:\X \rightarrow (0,1)$ by $\densityFunction(a)=\densityA$, $\densityFunction(c) = \volC$ and $\densityFunction(b) =\densityFunction(d)=1/3$. 


\begin{restatable}{lem}{propertiesCheckLemmaForUnknownNoiseLB}\label{propertiesCheckLemmaForUnknownNoiseLB} For $\twoMeasuresUnknownNoiseDistIndex \in \{0,1\}$ the measures $\Prob^{\twoMeasuresUnknownNoiseDistIndex}$ satisfy the following properties:
\begin{enumerate}[label=\alph*)]
    \item $\Prob^{\twoMeasuresUnknownNoiseDistIndex}$ satisfies Assumption \ref{classConditionalNoiseAssumption};
    \item $\Prob^{\twoMeasuresUnknownNoiseDistIndex}$ satisfies Assumption \ref{marginAssumption} parameters $(\marginExponent, \marginConstant)$ whenever $\marginConstant\geq 4^{\marginExponent}$ \& $\volC \leq \Delta^{\marginExponent}$;
    \item $\regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}$ satisfies Assumption \ref{holderAssumption} with parameters $(\holderExponent, \holderConstant)$ whenever $\Delta \leq \holderConstant \cdot r^{\holderExponent}$;
    \item $\marginalDistribution$ satisfies Assumption \ref{minimalMassAssumption} with parameters $(\dimensionExponent, \densityFunction)$ whenever $\volA \geq \densityA\cdot r^{\dimensionExponent}$;
    \item $\marginalDistribution$ satisfies Assumption \ref{tailAssumption} with parameters $(\tailsExponent, \tailsConstant, \tailsThreshold, \densityFunction)$ whenever $\tailsExponent \leq 1$, $\tailsThreshold \leq \frac{1}{3}$ \& $\volA \leq \densityA$;
    \item $\Prob^{\twoMeasuresUnknownNoiseDistIndex}$ satisfies Assumption \ref{quantitativeRangeAssumption} with parameters $(\fastLimitsExponent, \fastLimitsConstant,\fastLimitsThreshold,\densityFunction)$ whenever $\fastLimitsThreshold \leq 1/3$ \& $\Delta \leq \fastLimitsConstant \cdot \densityA^{\fastLimitsExponent}$. 
\end{enumerate}
\end{restatable}



\begin{proof} We check each property in turn.

\noindent Property \ref{classConditionalNoiseAssumption} follows immediately from the construction of $\Prob^{\twoMeasuresUnknownNoiseDistIndex}$ together with the fact that $\Delta <1/6$, so each $\probFlipFrom[j]^{\twoMeasuresUnknownNoiseDistIndex}<1/4$.

\noindent Property \ref{marginAssumption} follows from the fact that since $\Delta<1/6$, we have $\left|\regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(x)-1/2\right| \geq 1/3$ for $x \neq c$ and 
$\left|\regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(c)-1/2\right|\geq \Delta/4$. Property \ref{holderAssumption} follows from the fact that the only two distinct points $x_0, x_1$ with $\dist(x_0,x_1)<1$ are $a$ \& $b$ with $\dist(a,b)=r$ and $\left|\regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(a)-\regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(b)\right|\leq \Delta$.

\noindent Property \ref{minimalMassAssumption} follows from the fact that  $\marginalDistribution$ is defined by $\marginalDistribution(\{a\}) = \volA$, $\marginalDistribution(\{b\}) = 1/3$, $\marginalDistribution(\{c\}) = \volC$, $\marginalDistribution(\{d\}) = 2/3-\volA-\volC$ and $\densityFunction:\X \rightarrow (0,1)$ by $\densityFunction(a)=\densityA$, $\densityFunction(c) = \volC$ and $\densityFunction(b) =\densityFunction(d)=1/3$. In particular, for $x \neq a$ we have for $\tilde{r} \in (0,1)$ \[\marginalDistribution(B_{\tilde{r}}(x))\geq \marginalDistribution(\{x\}) \geq \densityFunction(x) \geq  \densityFunction(x) \cdot {\tilde{r}}^d.\]
On the other hand, for $x = a$ there are two cases. If ${\tilde{r}} \in (r,1)$ then \[\marginalDistribution(B_{\tilde{r}}(a))\geq \marginalDistribution(\{b\}) \geq 1/3 \geq \densityA \cdot {\tilde{r}}^{\dimensionExponent}=\densityFunction(a)\cdot {\tilde{r}}^{\dimensionExponent} \] since $\densityA <1/6$. If ${\tilde{r}}\leq r$ then $\marginalDistribution(B_{\tilde{r}}(a)) \geq \marginalDistribution(\{a\}) = \volA \geq \densityA \cdot r^d \geq \densityFunction(a)\cdot {\tilde{r}}^{\dimensionExponent}$.

\noindent Property \ref{tailAssumption} requires three cases. If $\epsilon \in [\max\{\densityA, \volC\},1/3)$ then we have
\[\marginalDistribution\left(\{x \in \X: \densityFunction(x)<\epsilon\}\right) =\marginalDistribution\left(\{a,c\}\right) = \volA+\volC \leq 2\max\{\densityA,\volC\} \leq \tailsConstant \cdot \epsilon^{\tailsExponent}.\]
If $\epsilon \in [\min\{\densityA, \volC\},\max\{\densityA, \volC\})$ then we take $x_0 \in \{a,c\}$ with $\densityFunction(x_0) = \min_{x \in \X}\{\densityFunction(x)\}$. Since $\volA \leq \densityA$ we have 
\[\marginalDistribution\left(\{x \in \X: \densityFunction(x)<\epsilon\}\right) =\marginalDistribution\left(\{x_0\}\right) \leq \densityFunction(x_0) = \min\{\densityA, \volC\}\leq \epsilon \leq \tailsConstant \cdot \epsilon^{\tailsExponent}.\]
Finally, for  $\epsilon \in (0,\min\{\densityA, \volC\})$ we have $\marginalDistribution\left(\{x \in \X: \densityFunction(x)<\epsilon\}\right)=0$.

\noindent Property \ref{quantitativeRangeAssumption} requires us to consider two cases. If $\epsilon \in [w, \fastLimitsThreshold)$ then since $\densityFunction(b) =\densityFunction(d)=1/3>\epsilon$ and for both $\twoMeasuresUnknownNoiseDistIndex \in \{0,1\}$ we have $\regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(b) \geq 1-\Delta$ and $\regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(d)=0$ we have 
\begin{align*}
\max\left\lbrace \inf_{x \in \suppMarginalDistribution}\left\lbrace \regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(x): \densityFunction(x) >\epsilon \right\rbrace, \inf_{x \in \suppMarginalDistribution}\left\lbrace 1-\regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(x): \densityFunction(x) >\epsilon \right\rbrace\right\rbrace \leq \Delta \leq \fastLimitsConstant \cdot \epsilon^{\fastLimitsExponent}.    
\end{align*}
On the other hand, if $\epsilon \in (0,w)$ then since $\densityFunction(a)=w$ and $\regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(a)=1$, and $\regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(d)=0$ we have
\begin{align*}
\max\left\lbrace \inf_{x \in \suppMarginalDistribution}\left\lbrace \regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(x): \densityFunction(x) >\epsilon \right\rbrace, \inf_{x \in \suppMarginalDistribution}\left\lbrace 1-\regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(x): \densityFunction(x) >\epsilon \right\rbrace\right\rbrace= 0 \leq \fastLimitsConstant \cdot \epsilon^{\fastLimitsExponent}.    
\end{align*}




\end{proof}









Recall that $\left(\noisy[\Prob]^{\twoMeasuresUnknownNoiseDistIndex}\right)^{\otimes n}$ is the product distribution with $\noisySample \sim \left(\noisy[\Prob]^{\twoMeasuresUnknownNoiseDistIndex}\right)^{\otimes n}$.

\begin{restatable}{lem}{KLBoundOnPairOfProductDistributionsLemma}\label{KLBoundOnPairOfProductDistributionsLemma} $\max\left\lbrace \kullbackLeiblerDivergence\left(\left(\noisy[\Prob]^{0}\right)^{\otimes n},\left(\noisy[\Prob]^{1}\right)^{\otimes n}\right),\kullbackLeiblerDivergence\left(\left(\noisy[\Prob]^{1}\right)^{\otimes n},\left(\noisy[\Prob]^{0}\right)^{\otimes n}\right)\right\rbrace \leq  n\cdot \volA \cdot (3\Delta/2)^2$.
\end{restatable}



\begin{proof} We shall show that $\kullbackLeiblerDivergence\left(\left(\noisy[\Prob]^{0}\right)^{\otimes n},\left(\noisy[\Prob]^{1}\right)^{\otimes n}\right)\leq n\cdot \volA \cdot (3\Delta/2)^2$. The proof that\\ $\kullbackLeiblerDivergence\left(\left(\noisy[\Prob]^{1}\right)^{\otimes n},\left(\noisy[\Prob]^{0}\right)^{\otimes n}\right)\leq n\cdot \volA \cdot (3\Delta/2)^2$ is similar. Recall that for each ${\twoMeasuresUnknownNoiseDistIndex}\in \{0,1\}$ we let $\noisy[\Prob]^{\twoMeasuresUnknownNoiseDistIndex}$ denote the marginal distribution of $\Prob^{\twoMeasuresUnknownNoiseDistIndex}$ over pairs $(X,\noisy[Y])$ consisting of a feature vector $X \sim \X$ and a corrupted label $\noisy[Y]\in \Y$. We can compute the corrupted regression functions $\noisyRegressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(x)= \Prob^{\twoMeasuresUnknownNoiseDistIndex}[\noisy[Y]|X=x]$ for ${\twoMeasuresUnknownNoiseDistIndex}\in \{0,1\}$ by applying (\ref{writingCorruptedRegressionFunctionInTermsOfRegressionFunctionEq}). Since $\probFlipZeroToOne^0=0$ and $\probFlipOneToZero^0=1/4$ we have $\noisyRegressionFunction^0(x) = (3/4)\cdot \regressionFunction^0(x)$ for all $x \in \X$. On the other hand, since $\probFlipZeroToOne^1=0$ and $\probFlipOneToZero^1=(1+3\Delta)/4$ we have $\noisyRegressionFunction^1(x) =(3/4)\cdot(1-\Delta)\cdot \regressionFunction^1(x)$ for all $x \in \X$.

We begin by bounding the  Kullback Leibler divergence between $\noisy[\Prob]^0$ and $\noisy[\Prob]^1$ using the fact that $\marginalDistribution(\{a\})=\volA$  and $\noisyRegressionFunction^0(x)=\noisyRegressionFunction^1(x)$ for $x \in \X \backslash \{a\}$,
\begin{align*}
\kullbackLeiblerDivergence\left(\noisy[\Prob]^{0},\noisy[\Prob]^{1}\right)& = \sum_{x \in \X}\sum_{y \in \Y} \noisy[\Prob]^0\left[X = x\hspace{2mm}\&\hspace{2mm}\noisy[Y]=y \right] \log \left(\frac{\noisy[\Prob]^0\left[X = x\hspace{2mm}\&\hspace{2mm}\noisy[Y]=y \right]}{\noisy[\Prob]^1\left[X = x\hspace{2mm}\&\hspace{2mm}\noisy[Y]=y \right]}\right)\\
& = \sum_{x \in \X} \marginalDistribution(\{x\}) \left( (1-\noisyRegressionFunction^0(x)) \log\left( \frac{1-\noisyRegressionFunction^0(x)}{1-\noisyRegressionFunction^1(x)}\right) + \noisyRegressionFunction^0(x)\log\left( \frac{\noisyRegressionFunction^0(x)}{\noisyRegressionFunction^1(x)}\right)
\right)\\
& = \volA \cdot \left( (1-\noisyRegressionFunction^0(a)) \log\left( \frac{1-\noisyRegressionFunction^0(a)}{1-\noisyRegressionFunction^1(a)}\right) + \noisyRegressionFunction^0(a)\log\left( \frac{\noisyRegressionFunction^0(a)}{\noisyRegressionFunction^1(a)}\right)
\right)\\
& \leq \volA \cdot \frac{\left(\noisyRegressionFunction^0(a)-\noisyRegressionFunction^1(a)\right)^2}{\min \left\lbrace \noisyRegressionFunction^0(a), (1-\noisyRegressionFunction^0(a)),\noisyRegressionFunction^1(a), 1-\noisyRegressionFunction^1(a)\right\rbrace}\leq  \volA \cdot (3\Delta/2)^2.
\end{align*}
The second to last inequality follows from the reverse Pinsker's inequality \cite[Lemma 6.3]{csiszar2006context}. The final inequality follows from the fact that $\noisyRegressionFunction^0(a) = 3/4$ and $\noisyRegressionFunction^0(a)=(3/4)\cdot (1-\Delta)$. Given that  $\left(\noisy[\Prob]^{\twoMeasuresUnknownNoiseDistIndex}\right)^{\otimes n}$ consists of $n$ independent copies of $\noisy[\Prob]^{\twoMeasuresUnknownNoiseDistIndex}$ for $\twoMeasuresUnknownNoiseDistIndex \in \{0,1\}$ we deduce that \[\kullbackLeiblerDivergence\left(\left(\noisy[\Prob]^{0}\right)^{\otimes n},\left(\noisy[\Prob]^{1}\right)^{\otimes n}\right)= n \cdot \kullbackLeiblerDivergence\left(\noisy[\Prob]^{0},\noisy[\Prob]^{1}\right) \leq n\cdot \volA \cdot (3\Delta/2)^2.\]

\end{proof}



\begin{lem}\label{applyingKLUpperBoundLemmaInPfOfLBWithUnknownNoiseLemma} Suppose that $2n\volA\cdot \Delta^2 \leq  1$. Given any $\noisySample$-measureable classifier $\classifier$ we have
\begin{align*}
\sum_{\twoMeasuresUnknownNoiseDistIndex \in \{0,1\}} \left( \ExpectationOverNoisySamples\left[ \risk\left(\classifier\right) \right] -  \risk\left(\oracle\right)  \right) \geq \frac{\volC\cdot \Delta}{24}.
\end{align*}
\end{lem}

\begin{proof} By Lemma \ref{KLBoundOnPairOfProductDistributionsLemma} combined with $2n\volA\Delta^2 \leq  1$ we have 
\[(2 \log 2)^{-1}\cdot\max\left\lbrace \kullbackLeiblerDivergence\left(\left(\noisy[\Prob]^{0}\right)^{\otimes n},\left(\noisy[\Prob]^{1}\right)^{\otimes n}\right),\kullbackLeiblerDivergence\left(\left(\noisy[\Prob]^{1}\right)^{\otimes n},\left(\noisy[\Prob]^{0}\right)^{\otimes n}\right)\right\rbrace \leq  \frac{3}{4}.\]
We construct an estimator $\hat{T}: \left(\X\times \Y\right)^n \rightarrow \left\lbrace \left(\noisy[\Prob]^{0}\right)^{\otimes n}, \left(\noisy[\Prob]^{1}\right)^{\otimes n}\right\rbrace$ in terms of an arbitrary classifier $\classifier$ as follows. Take $\hat{T}(\noisySample) = \left(\noisy[\Prob]^{\twoMeasuresUnknownNoiseDistIndex}\right)^{\otimes n}$ where $\twoMeasuresUnknownNoiseDistIndex=\classifier(c)$ and $\classifier$ is trained on $\noisySample$. Note that $\regressionFunction^0(c)<1/2$ and $\regressionFunction^1(c)>1/2$. Hence, for each $\Prob^{\twoMeasuresUnknownNoiseDistIndex}$ we have $\oracle(c)=\twoMeasuresUnknownNoiseDistIndex$ for the corresponding Bayes rule. By Birge's variant of Fano's lemma (Lemma \ref{birgesVersionOfFanosLemma}), we have
\begin{align}\label{lowerBoundExpectingCPointToBeNonBayesEq}
\sum_{\twoMeasuresUnknownNoiseDistIndex \in \{0,1\}}  \ExpectationOverNoisySamples\left[\one\left\lbrace \classifier(c) \neq \oracle(c) \right\rbrace  \right]  =\sum_{\twoMeasuresUnknownNoiseDistIndex \in \{0,1\}} \left(\noisy[\Prob]^{\twoMeasuresUnknownNoiseDistIndex}\right)^{\otimes n}\left[ \hat{T}\left( \noisySample\right) \neq \left(\noisy[\Prob]^{\twoMeasuresUnknownNoiseDistIndex}\right)^{\otimes n}\right] \geq \frac{1}{4},
\end{align}
where the expectation $\ExpectationOverNoisySamples$ is taken over all samples $\noisySample =\{ (X_i,\noisy[Y]_i)\}_{i \in [n]}$ with $\{ (X_i,Y_i,\noisy[Y]_i)\}_{i \in [n]}$ generated i.i.d. from $\Prob^{\twoMeasuresUnknownNoiseDistIndex}$. To complete the proof of the lemma we note that for both $\twoMeasuresUnknownNoiseDistIndex \in \{0,1\}$ we have $\left| 2\regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(c)-1\right| = \Delta/(2-\Delta) \geq \Delta/2$. Hence, for $\twoMeasuresUnknownNoiseDistIndex \in \{0,1\}$ and any $\decisionRule \in \setOfDecisionRules$ we have
\begin{align*}
\risk\left(\decisionRule\right) - \risk(\oracle) & = \int \left|2\regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(x)-1\right| \cdot \one \left\lbrace \decisionRule(x) \neq \oracle(x)\right\rbrace d\marginalDistribution(x)\\
& \geq \marginalDistribution(\{c\}) \cdot \left| 2\regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(c)-1\right| \cdot \one\left\lbrace \classifier(c) \neq \oracle(c) \right\rbrace\\ &\geq \volC \cdot\frac{\Delta}{2}\cdot \one\left\lbrace \classifier(c) \neq \oracle(c) \right\rbrace.
\end{align*}
Combining with (\ref{lowerBoundExpectingCPointToBeNonBayesEq}) completes the proof of the lemma.
\end{proof}

\paragraph{Proof of Proposition \ref{lowerBoundWithUnknownNoise}}  To prove the proposition we choose parameters $\left(\Delta,r, \volA, \volC,\densityA \right) \in (0,1/6)^5$ so as to maximise the lower bound $v\cdot \Delta/24$ whilst satisfying the conditions of Lemma \ref{propertiesCheckLemmaForUnknownNoiseLB} along with the condition $2nu \cdot \Delta^2 \leq 1$ from Lemma \ref{applyingKLUpperBoundLemmaInPfOfLBWithUnknownNoiseLemma}. We define $\Delta = 6^{-(1+\frac{1}{\marginExponent}+\fastLimitsExponent )} \cdot ({2n})^{-\frac{\fastLimitsExponent\holderExponent}{\fastLimitsExponent(2\holderExponent+\dimensionExponent)+\holderExponent}}$, $r = \Delta^{\frac{1}{\holderExponent}}$, $\volA = \Delta^{\frac{\holderExponent+\fastLimitsExponent \dimensionExponent}{\fastLimitsExponent \holderExponent}}$, $\volC = \Delta^{\marginExponent}$ and $\densityA=\Delta^{\frac{1}{\fastLimitsExponent}}$. It follows that $\left(\Delta,r, \volA, \volC,\densityA \right) \in (0,1/6)^5$. Moreover, one can then verify that the conditions of Lemma \ref{propertiesCheckLemmaForUnknownNoiseLB} hold, so for both $\twoMeasuresUnknownNoiseDistIndex \in \{0,1\}$ we have $\Prob^{\twoMeasuresUnknownNoiseDistIndex} \in \distributionClass\left(\Gamma\right)$. In addition, we have $2nu \cdot \Delta^2 \leq 1$, so by Lemma \ref{applyingKLUpperBoundLemmaInPfOfLBWithUnknownNoiseLemma},
\begin{align*}
\sup_{\Prob \in \distributionClass(\Gamma)} \left( \ExpectationOverNoisySamples\left[ \risk\left(\classifier\right) \right] -  \risk\left(\oracle\right)  \right) & \geq \frac{1}{2}\sum_{\twoMeasuresUnknownNoiseDistIndex \in \{0,1\}} \left( \ExpectationOverNoisySamples\left[ \risk\left(\classifier\right) \right] -  \risk\left(\oracle\right)  \right) \\
&\geq \frac{\volC\cdot \Delta}{48} = \frac{\Delta^{\marginExponent+1}}{48}= c_1 \cdot n^{-\frac{\fastLimitsExponent\holderExponent(\marginExponent+1)}{\fastLimitsExponent(2\holderExponent+\dimensionExponent)+\holderExponent}},
\end{align*}
where $c_1$ is determined by $\Gamma$. This completes the proof of the Proposition \ref{lowerBoundWithUnknownNoise}.
\QEDA

To complete the proof of Theorem \ref{mainMinimaxThmLowerBound} we will combine Proposition \ref{lowerBoundWithUnknownNoise} with Proposition \ref{lowerBoundWithKnownNoise} in the next section.

==> Archive/maximumEstimation.tex <==
In Section \ref{plugInCorruptedRegressionFunctionSec} we discussed how the noise probabilities $\probFlipZeroToOne$ and $\probFlipOneToZero$ are determined by the extrema of the corrupted regression function $\noisy[\regressionFunction]$. This motivates the question of determining the maximum of a function $f$, which is the focus of this section. As in Section \ref{KNNFuncEstSec}, we shall assume we have access to a sample $\sample_f = \left\lbrace \left(X_i,Z_i\right)\right\rbrace_{i \in [n]}$ with $(X_i,Z_i) \sim \Prob$ generated i.i.d. where $\Prob$ is an unknown distribution on $\X \times [0,1]$ with $f(x)= \E\left[Z|X=x\right]$. Our aim is to estimate $M(f):=\sup_{x \in \suppMarginalDistribution}\left\lbrace f(x) \right\rbrace$ based on $\sample_f$. In Section \ref{KNNMaxEstBoundedSubSec} we give a bound for a simple estimator in the setting of uniform smoothness. In Section \ref{KNNMaxEstUnboundedSubSec} we give a bound for an estimator for which applies more generally.

\subsection{Estimating the maximum of a function with uniform smoothness}\label{KNNMaxEstBoundedSubSec}

In this section we consider the following simple estimator for $M(f)$ based on $\KNNLepskiEst$ by
\begin{align*}
\empiricalMaximum[f] = \max_{i \in [n]}\left\lbrace \KNNLepskiEstBase{f}{n}{\delta/\left(2n\right)}\left(X_i\right)\right\rbrace.
\end{align*}


To bound the performance of $\empiricalMaximum[f]$ we require $f$ to be \emph{uniformly} measure-smooth.

\begin{defn}[Uniform measure-smoothness] A function $f:\X \rightarrow [0,1]$ is \emph{uniformly measure-smooth} with exponent $\measureSmoothnessExponent>0$ and constant $\measureSmoothnessConstant\geq 1$ if for all $x_0, x_1 \in \X$ we have $
\left|f(x_0)-f(x_1)\right|\leq \measureSmoothnessConstant \cdot \marginalDistribution\left(B_{\rho(x_0,x_1)}(x_0)\right)^{\measureSmoothnessExponent}$.
\end{defn}
Hence, a function $f$ is \emph{uniformly measure-smooth} with exponent $\measureSmoothnessExponent$ and constant $\measureSmoothnessConstant$ if $f$ is measure-smooth with a multiplier function $\localMeasureSmoothnessFactorFunction$ such that $\localMeasureSmoothnessFactorFunction(x) \leq \measureSmoothnessConstant$ for all $x \in \X$. We deduce the following bound from Corollary \ref{KNNPointwiseBoundLepskiChoiceKThm}.
\begin{theorem}[Maximum bound with uniform smoothness]\label{NaiveMaxBoundThm} Suppose that $f$ is \emph{uniformly measure-smooth} with exponent $\measureSmoothnessExponent>0$ and constant $\measureSmoothnessConstant$. Suppose further that $\sample_f$ is generated i.i.d. from $\Prob$. Then for any $n \in \N$ and $\delta \in \left(0,1\right)$ the following holds with probability at least $1-\delta$ over $\sample_f$,
\begin{align*}
\left| \empiricalMaximum[f]-M(f)\right| \leq  14 \cdot \measureSmoothnessConstant \cdot \left( \frac{\log(3n/\delta)}{n}\right)^{\frac{\measureSmoothnessExponent}{2\measureSmoothnessExponent+1}}.
\end{align*}
\end{theorem}
\begin{proof} The bound is trivial for $n=1$, so we may assume $n\geq 2$. By Corollary \ref{KNNPointwiseBoundLepskiChoiceKThm} combined with the union bound the following holds simultaneously for all $i \in [n]$, with probability at least $1-\delta/2$ over $\sample_f$,
\begin{align}\label{examplesAreCloseSimpleMaxThmEq}
\left| \KNNLepskiEstBase{f}{n}{\delta/\left(2n\right)}\left(X_i\right)-f(X_i)\right| &\leq 6\sqrt{2} \cdot \measureSmoothnessConstant^{\frac{1}{2\measureSmoothnessExponent+1}} \cdot \left( \frac{\log(3n^2/\delta)}{n}\right)^{\frac{\measureSmoothnessExponent}{2\measureSmoothnessExponent+1}}\\ \nonumber &\leq 12 \cdot \measureSmoothnessConstant \cdot \left( \frac{\log(3n/\delta)}{n}\right)^{\frac{\measureSmoothnessExponent}{2\measureSmoothnessExponent+1}}.
\end{align}
Here we use the fact that $f$ is \emph{uniformly measure-smooth} with constant $\measureSmoothnessConstant$. Now take $\epsilon>0$ and choose $x_0 \in \suppMarginalDistribution$ with $f(x_0)\geq M(f) -\epsilon$. In addition, take $p=\log(2/\delta)/n$, let $r_p(x_0) = \inf\left\lbrace r>0: \marginalDistribution\left(B_r(x_0)\right)\geq p\right\rbrace$ and let $B_0:= \left\lbrace x \in \X: \dist\left(x,x_0\right)\leq r_p(x_0)\right\rbrace = \bigcap_{r>r_p(x_0)}B_r(x_0)$. It follows that $\marginalDistribution\left(B_0\right)\geq p$. Hence, we have
\begin{align*}
\Prob_{\Xsample}\left[ \dist\left(X_{\tau_{n,1}(x_0)},x\right)>r_p(x_0) \right]& = \Prob_{\Xsample}\left[ \left\lbrace X_i\right\rbrace_{i \in [n]} \cap B_0 = \emptyset \right] \leq (1-p)^n\leq \exp(-n p) \leq 2^{-np}=\delta/2.
\end{align*}
Note that we can assume without loss of generality that $n \geq \log(3n/\delta)$ since otherwise the result is trivial. By the uniform measure-smoothness property we have 
\begin{align*}
\left|f(X_{\tau_{n,1}(x_0)}) - f(x_0)\right| & \leq  \measureSmoothnessConstant \cdot \marginalDistribution\left(B_{\rho(x_0,X_{\tau_{n,1}(x_0)})}(x_0)\right)^{\measureSmoothnessExponent} \leq  \measureSmoothnessConstant \cdot \marginalDistribution\left(B_{r_p(x_0)}(x_0)\right)^{\measureSmoothnessExponent} \\ & \leq \measureSmoothnessConstant \cdot p^{\measureSmoothnessExponent}  =   \measureSmoothnessConstant \cdot\left(\frac{\log(2/\delta)}{n}\right)^{\measureSmoothnessExponent} \leq \measureSmoothnessConstant \cdot \left( \frac{\log(3n/\delta)}{n}\right)^{\frac{\measureSmoothnessExponent}{2\measureSmoothnessExponent+1}}.
\end{align*}
Hence, with probability at least $1-\delta/2$ over $\sample_f$ we have
\begin{align*}
\max_{i \in [n]}\left\lbrace f(X_i)\right\rbrace \geq f(x_0)-\measureSmoothnessConstant \cdot \left( \frac{\log(3n/\delta)}{n}\right)^{\frac{\measureSmoothnessExponent}{2\measureSmoothnessExponent+1}} \geq M(f)-\measureSmoothnessConstant \cdot \left( \frac{\log(3n/\delta)}{n}\right)^{\frac{\measureSmoothnessExponent}{2\measureSmoothnessExponent+1}} -\epsilon.
\end{align*}
Since this holds for all $\epsilon>0$ we see that with probability at least $1-\delta/2$ over $\sample_f$,
\begin{align}\label{maxOfTrueFuncOnExamplesIsCloseToTrueMaxForSimpleMaxBoundEq}
M(f)-\measureSmoothnessConstant \cdot \left( \frac{\log(3n/\delta)}{n}\right)^{\frac{\measureSmoothnessExponent}{2\measureSmoothnessExponent+1}} \leq \max_{i \in [n]}\left\lbrace f(X_i)\right\rbrace  \leq M(f).
\end{align}
Combining \ref{maxOfTrueFuncOnExamplesIsCloseToTrueMaxForSimpleMaxBoundEq} with \ref{examplesAreCloseSimpleMaxThmEq} and taking the union bound completes the proof of the theorem.
\end{proof}

We now move to the difficult setting of non-uniform smoothness.


\subsection{Estimating the maximum of a function with non-uniform smoothness}\label{KNNMaxEstUnboundedSubSec}
Given a sample $\sample_f$, for each $\delta \in \left(0,1\right)$, $k \in [n]$ and $x \in \N$ we define
\begin{align*}
\KLLowerBoundKNN[f](x):=\inf\left\lbrace p \in [0,1]: k \cdot \KL\left(\KNNest[f](x) , p\right) \leq  \log((2n)^2/\delta) \right\rbrace.
\end{align*}
We then define $\maxEstNDelta:=\max_{(i,k) \in [n]^2}\left\lbrace \KLLowerBoundKNN[f](X_i) \right\rbrace$. Recall that a measure $\marginalDistribution$ is said to be doubling if there exists a constant $\doublingConstant[\marginalDistribution]\geq 1$ on $\X$ such that for each $x \in \suppMarginalDistribution$ and $r>0$ we have $\marginalDistribution\left(B_{2r}(x)\right)\leq \doublingConstant[\marginalDistribution]\cdot \marginalDistribution\left(B_r(x)\right)$. We have the following performance bound for $\maxEstNDelta$.

\begin{theorem}\label{functionMaximumEstimatorUnboundedSmoothnessTheorem}  Suppose that $\marginalDistribution$ is a doubling measure with doubling constant $\doublingConstant[\marginalDistribution]\geq 1$ and  $f:\X \rightarrow [0,1]$ is measure smooth with exponent $\measureSmoothnessExponent>0$ and multiplier function $\localMeasureSmoothnessFactorFunction:\X \rightarrow [1,\infty)$. Then with probability at least $1-\delta$ over $\sample$ we have
\begin{align}\label{functionMaximumEstimatorUnboundedSmoothnessTheoremConclusionEq}
\sup_{x \in \suppMarginalDistribution}\left\lbrace f(x)- 2^{4} \cdot \left(\doublingConstant[\marginalDistribution]^{2\measureSmoothnessExponent}\cdot\localMeasureSmoothnessFactor[x] \right)^{\frac{1}{2\measureSmoothnessExponent+1}}\cdot  \left(\frac{\log(2n/\delta)}{n} \right)^{\frac{\measureSmoothnessExponent}{2\measureSmoothnessExponent+1}}\right\rbrace \leq   \maxEstNDelta[f]\leq M(f).
\end{align}
\end{theorem}
Before proving Theorem \ref{functionMaximumEstimatorUnboundedSmoothnessTheorem} we give the following important corollaries.
\begin{corollary}[Consistency]\label{functionMaximumEstimatorUnboundedSmoothnessConsistentEstimatorCorollary} Suppose that the assumptions of Theorem \ref{functionMaximumEstimatorUnboundedSmoothnessTheorem} hold. Choose $\{\delta_n\}_{n \in \N}$ so that $\log(n/\delta_n)=o(n)$  and $\sum_{n \in \N}\delta_n<\infty$ (for example $\delta_n=1/n^2$). Then  $\maxEstNDeltaBase{f}{n}{\delta_n}$ is a consistent estimator of $M(f)$.
\end{corollary}
\begin{proof}[Proof of Corollary \ref{functionMaximumEstimatorUnboundedSmoothnessConsistentEstimatorCorollary}] By Theorem \ref{functionMaximumEstimatorUnboundedSmoothnessTheorem} combined with the Borel-Cantelli lemma the following holds with probability one,
\begin{align*}
M(f)&=\liminf_{n \rightarrow \infty}\left( \sup_{x \in \suppMarginalDistribution}\left\lbrace f(x)- 2^{4} \cdot \left(\doublingConstant[\marginalDistribution]^{2\measureSmoothnessExponent}\cdot\localMeasureSmoothnessFactor[x] \right)^{\frac{1}{2\measureSmoothnessExponent+1}}\cdot  \left(\frac{\log(2n/\delta)}{n} \right)^{\frac{\measureSmoothnessExponent}{2\measureSmoothnessExponent+1}}\right\rbrace\right)\\ &\leq \liminf_{n \rightarrow \infty}\left(  \maxEstNDelta[f]\right) \leq M(f).
\end{align*}
Here the first equality follows from the fact that $\log(n/\delta_n)=o(n)$.
\end{proof}
However, Corollary \ref{functionMaximumEstimatorUnboundedSmoothnessConsistentEstimatorCorollary} does not give us any information regarding the \emph{rate} of convergence. To obtain a bound on the rate of convergence we introduce the following condition which essentially says that the multiplier function $\localMeasureSmoothnessFactorFunction$ does not grow too quickly as $f$ approaches its maximum $M(f)$.

\begin{defn}[Fast limits]\label{fastLimitsDefn} A measure-smooth function $f:\X\rightarrow [0,1]$ with multiplier function $\localMeasureSmoothnessFactorFunction:\X\rightarrow [0,\infty)$ is said to satisfy the \emph{fast-limits} condition with exponent $\fastLimitsExponent>0$ and constants $\fastLimitsConstant,\fastLimitsLowerBoundConstant\geq 0$ if for all $t>\fastLimitsLowerBoundConstant$ we have
\[\sup_{x \in \suppMarginalDistribution}\left\lbrace f(x): \localMeasureSmoothnessFactor[x]\leq t \right\rbrace \geq M(f)-\fastLimitsConstant\cdot t^{-\fastLimitsExponent}.\]
\end{defn}
Note that a function $f$ which is uniformly measure-smooth with measure smoothness constant $\measureSmoothnessConstant$ will satisfy the fast-limits condition with any exponent $\fastLimitsExponent>0$ and any $\fastLimitsConstant\geq 0$, $\fastLimitsLowerBoundConstant= \measureSmoothnessConstant$. Given the fast limits condition we have the following rate of convergence.
\begin{corollary}[Fast limits bound]\label{functionMaximumEstimatorWithFastLimitsCondition} Suppose that in addition to the assumptions of Theorem \ref{functionMaximumEstimatorUnboundedSmoothnessTheorem}, the function $f$ satisfies the fast-limits condition with  exponent $\fastLimitsExponent>0$ and constants $\fastLimitsConstant,\fastLimitsLowerBoundConstant\geq 0$. Choose $\delta \in \left(0,1\right)$ and $n\in \N$ sufficiently large that $n/\log(2n/\delta) \geq \fastLimitsLowerBoundConstant^{\frac{1+\fastLimitsExponent(2\measureSmoothnessExponent+1)}{\measureSmoothnessExponent}}$. Then with probability at least $1-\delta$ over $\sample$ we have
\begin{align*}
\left|  \maxEstNDelta[f]- M(f)\right| \leq \left(\fastLimitsConstant+2^4\cdot \doublingConstant[\marginalDistribution]^{\frac{2\measureSmoothnessExponent}{2\measureSmoothnessExponent+1}}\right) \cdot \left(\frac{\log(2n/\delta)}{n}\right)^{\frac{\fastLimitsExponent \measureSmoothnessExponent}{1+\fastLimitsExponent(2\measureSmoothnessExponent+1)}}.
\end{align*}
\end{corollary}
\begin{proof} First apply Theorem \ref{functionMaximumEstimatorUnboundedSmoothnessTheorem} and then apply the fast limits condition with $t = \left(n/\log(2n/\delta)\right)^{\frac{\measureSmoothnessExponent}{1+\fastLimitsExponent(2\measureSmoothnessExponent+1)}}$.
\end{proof}


We now turn to the proof of Theorem \ref{functionMaximumEstimatorUnboundedSmoothnessTheorem}. To prove Theorem \ref{functionMaximumEstimatorUnboundedSmoothnessTheorem} we require two lemmas. For each $x \in \X$ and $k \in [n]$ we let $\conditionalExpectKNNest[f](x)=\frac{1}{k} \cdot \sum_{q \in [k]}f\left(X_{\tau_{n,q}(x)}\right)$.

\begin{lemma}\label{klLBIsWellBehavedForNonUniformMaxLemma} With probability at least $1-\delta/2$ over $\sample_f$, the following holds simultaneously for all $(i,k) \in [n]^2$,
\begin{align}\label{klLBIsWellBehavedForNonUniformMaxLemmaConclusionEq}
\conditionalExpectKNNest[f](X_i)-  \sqrt{2\log((2n)^2/\delta)/k} \leq \KLLowerBoundKNN[f](X_i) \leq \conditionalExpectKNNest[f](X_i).  
\end{align}
\end{lemma}
The proof of Lemma \ref{klLBIsWellBehavedForNonUniformMaxLemma} is given in \ref{proofOfKLLowerConfidenceBoundLemmaSec}. Define for $x\in \X$ and $p \in [0,1]$, $r_p(x) = \inf\left\lbrace r>0: \marginalDistribution\left(B_r(x)\right)\geq p\right\rbrace$.
\begin{restatable}{lemma}{closeNeighboursFixedPointLemma}\label{closeNeighboursFixedPointLemma} Take $x \in \X$, $k \in [n]$ and $p\in [k/n,1]$. Then
\begin{align*}
\Prob_{\sample}\left[ \rho\left(x,X_{\tau_{n,k}(x)}\right) > r_p(x)\right] \leq \exp\left(-\frac{k}{2}\cdot\left(1-\frac{k}{np}\right)^2\right).
 \end{align*}
\end{restatable}
Lemma \ref{closeNeighboursFixedPointLemma} follows from the multiplicative Chernoff bound. The proof is given in \ref{standardLemmasProofSec}. We now complete the proof of Theorem \ref{functionMaximumEstimatorUnboundedSmoothnessTheorem}.

\newcommand{\deterministicUncertainty}{u}

\begin{proof}[Proof of Theorem \ref{functionMaximumEstimatorUnboundedSmoothnessTheorem}] For the purpose of the proof we shall write $\deterministicUncertainty(x):=2^{4} \cdot \left(\doublingConstant[\marginalDistribution]^{2\measureSmoothnessExponent}\cdot\localMeasureSmoothnessFactor[x] \right)^{\frac{1}{2\measureSmoothnessExponent+1}}\cdot  \left(\frac{\log(2n/\delta)}{n} \right)^{\frac{\measureSmoothnessExponent}{2\measureSmoothnessExponent+1}}$ for $x \in \X$. By Lemma \ref{klLBIsWellBehavedForNonUniformMaxLemma} combined with the union bound it suffices to show that (\ref{functionMaximumEstimatorUnboundedSmoothnessTheoremConclusionEq}) holds with probability at least $1-\delta/2$,  whenever (\ref{klLBIsWellBehavedForNonUniformMaxLemmaConclusionEq}) holds. Hence, we shall assume that (\ref{klLBIsWellBehavedForNonUniformMaxLemmaConclusionEq}) holds. It follows immediately that  
\begin{align*}
\maxEstNDelta[f]\leq \max_{(i,k) \in [n]^2}\left\lbrace \conditionalExpectKNNest[f](X_i) \right\rbrace\leq \sup_{x \in \suppMarginalDistribution}\left\lbrace f(x)\right\rbrace
\end{align*}
Thus, we must show that $\maxEstNDelta[f] \geq \sup_{x \in \suppMarginalDistribution}\left\lbrace f(x)-\deterministicUncertainty(x)\right\rbrace$ with probability at least $1-\delta/2$. We shall also assume that there exists some $x \in \suppMarginalDistribution$ with $f(x)-\deterministicUncertainty(x)>0$. If this is not the case then the result is trivial since $\maxEstNDelta[f]\geq 0$.  Now take any $t \in \left(0, \sup_{x \in \suppMarginalDistribution}\left\lbrace f(x)-\deterministicUncertainty(x)\right\rbrace\right)$ and choose some $x_0 \in \suppMarginalDistribution$ with $f(x_0)-\deterministicUncertainty(x_0)>t$. Take $k:= \left\lceil \left(\left({2^{1-4\measureSmoothnessExponent}\cdot \log((2n)/\delta)}\right)/\left({\doublingConstant[\marginalDistribution]^{4\measureSmoothnessExponent}\cdot \localMeasureSmoothnessFactor[x]^2}\right)\right) \cdot n^{\frac{2\measureSmoothnessExponent}{2\measureSmoothnessExponent+1}} \right\rceil$. Since $f(x_0)-\deterministicUncertainty(x_0)>0$ we have $\deterministicUncertainty(x_0)<1$ which implies $k\geq 8 \log((2n)/\delta)\geq 1$. Hence,
\begin{align*}
\left(\frac{2^{1-4\measureSmoothnessExponent}\cdot \log((2n)/\delta)}{\doublingConstant[\marginalDistribution]^{4\measureSmoothnessExponent}\cdot \localMeasureSmoothnessFactor[x]^2}\right) \cdot n^{\frac{2\measureSmoothnessExponent}{2\measureSmoothnessExponent+1}}\leq k \leq \left(\frac{2^{2-2\measureSmoothnessExponent}\cdot \log((2n)/\delta)}{\doublingConstant[\marginalDistribution]^{4\measureSmoothnessExponent}\cdot \localMeasureSmoothnessFactor[x]^2}\right) \cdot n^{\frac{2\measureSmoothnessExponent}{2\measureSmoothnessExponent+1}}.
\end{align*}
Now choose $i_0 =\tau_{n,1}(x_0)$. By (\ref{klLBIsWellBehavedForNonUniformMaxLemmaConclusionEq}) we have
\begin{align}\label{varPartOfFunctionMaximumEstimatorUnboundedSmoothnessTheoremEq}
\maxEstNDelta[f] &= \max_{(i,q) \in [n]^2}\left\lbrace \KLLowerBoundKNNBase{f}{n}{q}{\delta}(X_i)\right\rbrace \geq \KLLowerBoundKNNBase{f}{n}{k}{\delta}(X_{i_0}) \\ \nonumber &\geq \conditionalExpectKNNest[f](X_{i_0})-\sqrt{2\log((2n)^2/\delta)/k}\\ \nonumber
&\geq \conditionalExpectKNNest[f](X_{i_0})- 2^{3} \cdot \left(\doublingConstant[\marginalDistribution]^{2\measureSmoothnessExponent}\cdot\localMeasureSmoothnessFactor[x] \right)^{\frac{1}{2\measureSmoothnessExponent+1}}\cdot  \left(\frac{\log(2n/\delta)}{n} \right)^{\frac{\measureSmoothnessExponent}{2\measureSmoothnessExponent+1}}\\ \nonumber &\geq \conditionalExpectKNNest[f](X_{i_0}) - \frac{1}{2}\cdot \deterministicUncertainty(x_0). 
\end{align}
Now take $p=(2k)/n$. By Lemma \ref{closeNeighboursFixedPointLemma} combined with the fact that $k\geq 8 \log((2n)/\delta) \geq 8 \log(2/\delta)$ we have
\begin{align*}
\Prob_{\sample}\left[ \rho\left(x_0,X_{\tau_{n,k}(x_0)}\right) > r_p(x_0)\right] \leq \exp\left(-\frac{k}{2}\cdot\left(1-\frac{k}{np}\right)^2\right) \leq \delta/2.
 \end{align*}
Hence, $\max_{q \in [k]}\left\lbrace \rho\left(x_0,X_{\tau_{n,q}(x_0)}\right) \right\rbrace =  \rho\left(x_0,X_{\tau_{n,k}(x_0)}\right) \leq r_p(x)$ holds with probability at least $1-\delta/2$. In particular, this implies that $\rho\left(x_0,X_{i_0}\right) \leq r_p(x_0)$. By the triangle, inequality we have $\rho\left(X_{i_0},X_{\tau_{n,q}(x_0)}\right) \leq 2\cdot r_p(x)$ for $q \in [k]$. Hence, we must have $\rho\left(X_{i_0},X_{\tau_{n,q}(X_{i_0})}\right) \leq 2\cdot r_p(x)$ for $q \in [k]$. Applying the triangle inequality once more we infer that  $\rho\left(x_{0},X_{\tau_{n,q}(X_{i_0})}\right) \leq 3\cdot r_p(x)$ for $q \in [k]$. Hence, by the measure smoothness property and the doubling property we see that for each $q \in [k]$,
\begin{align*}
\left|f\left(X_{\tau_{n,q}(X_{i_0})}\right)-f(x_0)\right|&\leq \localMeasureSmoothnessFactor[x_0] \cdot \marginalDistribution\left(B_{3\cdot r_p(x_0)}(x_0)\right)^{\measureSmoothnessExponent} 
\leq \left(\localMeasureSmoothnessFactor[x_0] \cdot \doublingConstant[\marginalDistribution]^{2\measureSmoothnessExponent}\right)\cdot \marginalDistribution\left(B_{r_p(x_0)}(x_0)\right)^{\measureSmoothnessExponent}\\&\leq \left(\localMeasureSmoothnessFactor[x_0] \cdot \doublingConstant[\marginalDistribution]^{2\measureSmoothnessExponent}\right)\cdot p^{\measureSmoothnessExponent}= 2^{\measureSmoothnessExponent}\cdot \left(\localMeasureSmoothnessFactor[x_0] \cdot \doublingConstant[\marginalDistribution]^{2\measureSmoothnessExponent}\right)\cdot \left(\frac{k}{n}\right)^{\measureSmoothnessExponent} \leq \frac{1}{2}\cdot \deterministicUncertainty(x_0).
\end{align*}
This implies $\conditionalExpectKNNest[f](X_{i_0})\geq f(x_0)-(1/2)\cdot \deterministicUncertainty(x_0)$.
By combining with (\ref{varPartOfFunctionMaximumEstimatorUnboundedSmoothnessTheoremEq}) we see that $\maxEstNDelta[f]\geq f(x_0)-\deterministicUncertainty(x_0)>t$ holds with probability at least $1-\delta/2$. Since this holds for all $t\in\left(0, \sup_{x \in \suppMarginalDistribution}\left\lbrace f(x)-\deterministicUncertainty(x)\right\rbrace\right)$, we deduce that with probability at least $1-\delta/2$ we have $\maxEstNDelta[f]\geq\sup_{x \in \suppMarginalDistribution}\left\lbrace f(x)-\deterministicUncertainty(x)\right\rbrace$. This completes the proof of the theorem.
\end{proof}

==> Archive/oldNotes.tex <==
Need to discuss findings
 - compare with other papers
 - what do the main theorems mean (eg. compare with minimax l.b.s)
 
 Argue for assumptions (natural, exponents don't need to be known)
 
 Compare with Cannings and Gadat's choice of k..
 
Sections:

Intro
Problem setup
Inconsistency
Main assumptions and related work in noiseless setting
Plug in method
K NN for function estimation
General KNN bound
Consistency
Global smoothness (now with standard k-nn ie. not Lepski)
Local smoothness
Empirical section
Discussion




How about:


Intro
Problem setup
- Plug in method
- K NN for function estimation [if no Lepski in the global smoothness section then should this move into those sectiore] - Agreed :)

Inconsistency of kNN

General KNN bound [? not sure what this is? - Something like Theorem 1 in Chaudhuri & Dasgupta - we give a bound which implies both the consistency and the finite sample results] [with or without label noise? - with - that would be the difference ie. with label noise & with the corresponding change in the KNN method] [what's the difference between this and the Global Smoothness section?] [Three differences: 1. No Lepski - Standard KNN based approach (with label noise adjustment), 2. More general (not assuming continuity at this stage), 3. Doesn't give the best rates in the global smoothness case (we need the lepski stuff for that)]
Consistency
Main assumptions and related work in noiseless setting

Global smoothness (now with standard k-nn ie. not Lepski)
Local smoothness
Empirical section
Discussion



==> Archive/plugInMethodCorruptedRegressionFunction.tex <==
The `plug-in' classification method is inspired by the fact that the mapping $\oracle:\X\rightarrow \Y$ for $x \in \X$ defined by $\oracle(x) = \one\left\lbrace \regressionFunction(x)\geq 1/2\right\rbrace$ is a Bayes classifier and minimises the risk $\risk(\classifier)$ over all measurable classifiers $\classifier:\X\rightarrow\Y$. We proceed by first producing an estimate $\est[\regressionFunction]:\X\rightarrow [0,1]$ of the regression function $\regressionFunction$ and then taking $\est[\classifier](x):=\one\left\lbrace \est[\regressionFunction](x)\geq 1/2\right\rbrace$. To apply this method in the label-noise setting we must first give a method for constructing an estimate $\est[\regressionFunction]$ based upon the corrupted sample $\noisy[\sample]$. By (\ref{noisyRegInTermsOfTrueRegEq}) for each $x \in \X$ we have
\begin{align}\label{trueRegInTermsOfNoisyRegEq}
\regressionFunction(x)=\left(1-\probFlipZeroToOne-\probFlipOneToZero\right)^{-1}\cdot\left(\noisy[\regressionFunction](x)-\probFlipZeroToOne\right)
\end{align}
We can construct an estimator $\noisy[{\est[\regressionFunction]}]$ for the corrupted regression function $\noisy[\regressionFunction]$ based upon the corrupted sample $\noisy[\sample]$ by using supervised regression methods (see Section ???). The key remaining challenge is to obtain estimates $\estProbFlipZeroToOne$ and $\estProbFlipOneToZero$ for $\probFlipZeroToOne$ and $\probFlipOneToZero$, respectively. Without further assumptions this is not possible (see \cite[Section 4]{scott2013classification}). Following \cite{menon2015learning} and \cite{scott2013classification} we make the following assumption on the range of the regression function.
\begin{assumption}[Range assumption]\label{rangeAssumption} We have $\inf_{x \in \suppMarginalDistribution}\left\lbrace \regressionFunction(x) \right\rbrace=0$ and $\sup_{x \in \suppMarginalDistribution}\left\lbrace \regressionFunction(x) \right\rbrace=1$.
\end{assumption}
By combining Assumption \ref{rangeAssumption} with (\ref{noisyRegInTermsOfTrueRegEq}) we have $\inf_{x \in \suppMarginalDistribution}\left\lbrace \noisy[\regressionFunction](x) \right\rbrace=\probFlipZeroToOne$ and $\sup_{x \in \suppMarginalDistribution}\left\lbrace \noisy[\regressionFunction](x) \right\rbrace=1-\probFlipOneToZero$. Hence, we may obtain estimates $\estProbFlipZeroToOne$ and $\estProbFlipOneToZero$ by estimating the extrema of the corrupted regression function $\noisy[\regressionFunction]$. This leads to the following `plug-in' template for classification based upon the corrupted regression function (Algorithm \ref{classificationBasedOnCorruptedRegressionFunctionAlgo}).


\begin{algorithm}[htbp]
%\floatconts
%{alg:KNNInd}
 {\caption{The plug-in method with label noise\label{classificationBasedOnCorruptedRegressionFunctionAlgo}}}
{ 
 \begin{enumerate}
     \item Compute an estimate $\noisy[{\est[\regressionFunction]}]$ of the corrupted regression function $\noisy[\regressionFunction]$ based on $\noisy[\sample]$;
     \item Compute $\estProbFlipZeroToOne$ and $\estProbFlipOneToZero$ by estimating the extrema of $\noisy[\regressionFunction]$ based on $\noisy[\sample]$;
     \item Let $\est[\classifier](x):= \one\left\lbrace \noisy[{\est[\regressionFunction]}](x) \geq 1/2 \cdot \left(1+\estProbFlipZeroToOne-\estProbFlipOneToZero\right) \right\rbrace$.
     \end{enumerate}
 }
\end{algorithm}
We shall use $k$-nearest neighbour methods to estimate the corrupted regression function $\noisy[\regressionFunction]$ based on $\noisy[\sample]$.



==> Archive/problemStatementNotation.tex <==

Suppose we have a feature space $\X$ with a metric $\dist$ and set of labels $\Y = \{0,1\}$. Let $\Prob$ be a fixed but unknown distribution on $\X \times \Y$.  Our goal is to learn a classifier $\classifier:\X \rightarrow \Y$ which minimises the risk
\begin{align*}
\risk\left(\classifier\right):= \E\left[ \classifier(X) \neq Y \right].
\end{align*}
Our data will be generated by a \emph{corrupted} distribution $\noisy[\Prob]$ on $\X\times \Y$ with asymmetric label noise. We shall assume a model of feature independent label noise, so there exists probabilities $\probFlipZeroToOne, \probFlipOneToZero \in \left(0,1\right)$ with $\probFlipZeroToOne+\probFlipOneToZero<1$ such that random pairs $(X,\noisy[Y])\sim \noisy[\Prob]$ are generated by $(X,Y) \sim \Prob$ and $\noisy[Y]\neq Y$ with probability $\probFlipFrom[Y]$ and $\noisy[Y]=Y$ otherwise. We have access to a data set $\noisySample = \left\lbrace \left(X_i,\noisy[Y]_i\right)\right\rbrace_{i \in [n]}$ consisting independent and identically distributed pairs generated from the corrupted distribution $\left(X_i,\noisy[Y]_i\right) \sim \noisy[\Prob]$.


We let $\marginalDistribution$ denote the  marginal distribution over the features i.e. $\marginalDistribution(A) = \Prob\left[ X \in A \right]$ for Borel sets $A \subset \X$, and let $\regressionFunction:\X\rightarrow [0,1]$ denote the regression function i.e. $\regressionFunction(x) = \Prob\left[ Y=1 | X=x\right]$. We also let $\suppMarginalDistribution\subseteq \X$ denote the support of $\marginalDistribution$. It follows from the assumption of feature independent label noise that the corrupted distribution $\noisy[\Prob]$ has the same marginal distribution $\Prob$ ie. $\noisy[\Prob]\left[ X \in A \right]= \marginalDistribution\left(A\right)$ for $A \subset \X$. Moreover, if we let $\noisy[\regressionFunction]:\X\rightarrow [0,1]$ denote the corrupted regression function $\noisy[\regressionFunction](x)  = \noisy[\Prob]\left[\noisy[Y]=1|X=x\right]$, then $\noisy[\regressionFunction]$ and $\regressionFunction$ are related by
\begin{align}\label{noisyRegInTermsOfTrueRegEq}
\noisy[\regressionFunction](x) = \left(1-\probFlipOneToZero\right) \cdot \Prob\left[Y=1|X=x\right] + \probFlipZeroToOne \cdot \Prob\left[Y=0|X=x\right]=\left(1-\probFlipZeroToOne-\probFlipOneToZero\right) \cdot \regressionFunction(x)+\probFlipZeroToOne.
\end{align}
We shall use this connection to provide a classifier based upon the corrupted regression function.



==> completingMinimaxThm.tex <==


\section{Completing the proof of Theorem \ref{mainMinimaxThm}}\label{completingMinimaxThmSec}




\paragraph{Proof of Theorem \ref{mainMinimaxThm}} The proof of Theorem \ref{mainMinimaxThm} requires a lower bound and upper bound. We begin with the lower bound. In Section \ref{mainLBSec} we proved
\begin{align*}
\inf_{\classifier}\left\lbrace \sup_{\Prob \in \distributionClass(\Gamma)}\left\lbrace\ExpectationOverNoisySamples\left[ \risk\left(\classifier\right) \right] -  \risk\left(\oracle\right) \right\rbrace\right\rbrace &\geq c_1 \cdot n^{-\frac{\fastLimitsExponent \holderExponent(\marginExponent+1)}{\fastLimitsExponent(2\holderExponent+\dimensionExponent)+\holderExponent}}.
\end{align*}
Moreover, Proposition \ref{lowerBoundWithKnownNoise} in Appendix \ref{LBForUncorruptedDataAppendix} is equivalent to
\begin{align*}
\inf_{\classifier}\left\lbrace \sup_{\Prob \in \distributionClass(\Gamma)}\left\lbrace
\ExpectationOverNoisySamples\left[ \risk\left(\classifier\right) \right] -  \risk\left(\oracle\right) \right\rbrace\right\rbrace& \geq c_0 \cdot n^{-\frac{\holderExponent \tailsExponent(\marginExponent+1)}{\tailsExponent(2\holderExponent+\dimensionExponent)+\marginExponent\holderExponent} },
\end{align*}
Combining these two lower bounds gives the lower bound in Theorem \ref{mainMinimaxThm}. To prove the upper bound we simply apply Theorem \ref{mainUpperBoundThm} in Section \ref{mainUpperBoundThmSec} (proved in Appendix \ref{proofOfHPUpperBoundAppendix}), with \[\delta_n = \min\left\lbrace n^{-\frac{\fastLimitsExponent \holderExponent(\marginExponent+1)}{\fastLimitsExponent(2\holderExponent+\dimensionExponent)+\holderExponent}},  n^{-\frac{\holderExponent \tailsExponent(\marginExponent+1)}{\tailsExponent(2\holderExponent+\dimensionExponent)+\marginExponent\holderExponent} }\right\rbrace.\]






\QEDA

==> oldMaxEstimationSec.tex <==

\section{A lower confidence bound approach to function maximisation}\label{funcMaxSec}

SAY MORE HERE ??????

We define 
\begin{align}\label{estOfFunctionMaxDef}
\hat{M}_{n,\delta}(f):= \max_{(i,k) \in [n]^2}\left\lbrace \hat{f}_{n,k}(X_i)-\sqrt{\frac{\log(4n/\delta)}{k}}\right\rbrace .
\end{align}


????


\begin{theorem}\label{funcMaxThm} Suppose that $f$ satisfies the H\"{o}lder assumption with parameters $(\holderExponent, \holderConstant)$ and $\marginalDistribution$ satisfies the minimal mass assumption with parameters $(\dimensionExponent, \densityFunction)$. Given any $n \in \N$ and $\delta \in (0,1)$ with probability at least $1-\delta$ over $\sample_f$ we have
\begin{align}\label{ineqsForFuncMaxThm}
\sup_{x \in \suppMarginalDistribution}\left\lbrace f(x) -7 \cdot   {\holderConstant}^{\frac{\dimensionExponent}{2\holderExponent+\dimensionExponent}} \cdot\left( \frac{\log(4n/\delta)}{\densityFunction(x)\cdot n} \right)^{\frac{\holderExponent}{2\holderExponent+\dimensionExponent}}\right\rbrace \leq \hat{M}_{n,\delta}(f) \leq M(f).
\end{align}
\end{theorem}

We require two lemmas which also play a role in the proof of Theorem \ref{knnRegressionBoundLepskiK}.

\begin{lem}\label{closeNeighboursLemma} Suppose that $\marginalDistribution$ satisfies the minimal mass assumption with parameters $(\dimensionExponent, \densityFunction)$. Given any $n \in \N$, $\delta \in (0,1)$, $x \in \X$ and $k \in \N \cap [8 \log(1/\delta), \densityFunction(x) \cdot (n/2)]$, with probability at least $1-\delta$ over $\sample_f$ we have
$\dist\left(x,X_{\tau_{n,k}(x)}\right)< \left( {2k}/\left({\densityFunction(x) \cdot n}\right) \right)^{\frac{1}{\dimensionExponent}}$.
\end{lem}
The proof of Lemma \ref{closeNeighboursLemma} is similar to \cite[Lemma 8]{chaudhuri2014rates}. Lemma \ref{closeNeighboursLemma} . Let $\bm{X}=\left\lbrace X_i\right\rbrace_{i \in [n]}$, $\bm{Z}=\left\lbrace Z_i\right\rbrace_{i \in [n]}$ and $\Prob_{\bm{Z}|\bm{X}}$ denote the conditional probability over $\bm{Z}$, conditioned on $\bm{X}$, with $(X_i,Z_i) \sim \Prob_f$. 

\begin{lem}\label{knnEstIsCloseToItsConditionalExpectationLemma} For all $n \in \N$, $\delta \in (0,1)$, $x \in \X$, $\bm{X} \in \X^n$ and $k \in [n]$ we have \[\Prob_{\bm{Z}|\bm{X}}\left[
\left|  \hat{f}_{n,k}(x)- \E_{\bm{Z}|\bm{X}}\left[\hat{f}_{n,k}(x)\right]\right| \geq \sqrt{\frac{\log(2/\delta)}{2k}}\right] \leq \delta.\]
\end{lem}
 Lemma \ref{knnEstIsCloseToItsConditionalExpectationLemma} is a consequence of Hoeffding's inequality.  A full proof of both lemmas is given in Appendix \ref{proofOfKNNRegressionBoundsAppendix}.



\begin{proof}
It suffices to show that for any fixed point $x_0 \in \X$ the following holds with probability at least $1-\delta$ over $\sample_f$ we have
\begin{align}\label{toProveInMaxThmBound}
 f(x_0) -7 \cdot   {\holderConstant}^{\frac{\dimensionExponent}{2\holderExponent+\dimensionExponent}} \cdot\left( \frac{\log(4n/\delta)}{\densityFunction(x_0)\cdot n} \right)^{\frac{\holderExponent}{2\holderExponent+\dimensionExponent}} \leq \hat{M}_{n,\delta}(f) \leq M(f).
\end{align}
Indeed, the bound (\ref{ineqsForFuncMaxThm}) may then be deduced by continuity of measure.


?????REPHRASE \& Rarrange - put the upper bound first!! ???? As in the proof of Theorem \ref{knnRegressionBoundLepskiK} we may choose $\tilde{k} \in \N$ with $8\log(2n/\delta)\leq \tilde{k}\leq \densityFunction(x_0)\cdot n/2$ and
\begin{align}\label{tildeKBoundForMaxThm}
\frac{1}{4} \cdot \left(\densityFunction(x_0)\cdot n\right)^{\frac{2\holderExponent}{2\holderExponent+\dimensionExponent}} \cdot \left(\frac{ \log(4n/\delta)}{\holderConstant^2}\right)^{\frac{\dimensionExponent}{2\holderExponent+\dimensionExponent}}\leq \tilde{k} \leq \frac{1}{2} \cdot \left(\densityFunction(x_0)\cdot n\right)^{\frac{2\holderExponent}{2\holderExponent+\dimensionExponent}} \cdot \left(\frac{ \log(4n/\delta)}{\holderConstant^2}\right)^{\frac{\dimensionExponent}{2\holderExponent+\dimensionExponent}}.
\end{align} 
By Lemma \ref{closeNeighboursLemma}, combined with the upper bound in (\ref{tildeKBoundForMaxThm}), the following holds with probability at least $1-\delta/2$ over $\sample_f$
\begin{align}\label{closeNeighboursAppInMaxThmPf}
\dist\left(x_0,X_{\tau_{n,\tilde{k}}(x)}\right)< \left( \frac{2\tilde{k}}{\densityFunction(x_0) \cdot n} \right)^{\frac{1}{\dimensionExponent}} \leq \xi:=\left(\frac{\log(4n/\delta)}{\holderConstant^2 \cdot \densityFunction(x_0) \cdot n}\right)^{\frac{1}{2\holderExponent+\dimensionExponent}}.
\end{align}
By Lemma \ref{knnEstIsCloseToItsConditionalExpectationLemma} combined with the union bound the following holds simultaneously over all pairs $(i,k) \in [n]^2$ with probability at least $1-\delta/2$,
\begin{align}\label{conditionalExpectationApplicationBoundInMaxThmPf}
\left|  \hat{f}_{n,k}(X_i)- \E_{\bm{Z}|\bm{X}}\left[\hat{f}_{n,k}(X_i)\right]\right| < \sqrt{\frac{\log(2/(\delta/(2n^2))}{2k}}\leq \sqrt{\frac{\log(4n/\delta)}{k}}.
\end{align}
Let's assume that (\ref{closeNeighboursAppInMaxThmPf}) and (\ref{conditionalExpectationApplicationBoundInMaxThmPf}) hold. By the union bound this is the case with probability at least $1-\delta$. Now take $i_0 =\tau_{n,1}(x_0) \in [n]$. By (\ref{closeNeighboursAppInMaxThmPf}) combined with the triangle inequality, for each $q \in [\tilde{k}]$ we have
\begin{align}
\dist\left(X_{i_0},X_{\tau_{n,q}(x)}\right) \leq \dist\left(x_0,X_{i_0}\right)+\dist\left(x_0,X_{\tau_{n,q}(x)}\right) \leq 2\cdot\xi,
\end{align}
where $\xi$ is defined in (\ref{closeNeighboursAppInMaxThmPf}). Hence, for each $q \in [\tilde{k}]$ we have $\dist\left(X_{i_0},X_{\tau_{n,q}(X_{i_0})}\right)\leq 2\cdot \xi$. Applying  (\ref{closeNeighboursAppInMaxThmPf}) once again we see that for all $q \in [\tilde{k}]$ 
\begin{align*}
\dist\left(x_0,X_{\tau_{n,q}(X_{i_0})}\right) \leq \dist\left(x_0,X_{i_0}\right)+\dist\left(X_{i_0},X_{\tau_{n,q}(X_{i_0})}\right) \leq 3\cdot \xi.
\end{align*}
By the H\"{o}lder assumption we deduce that 
\begin{align*}
\left| \E_{\bm{Z}|\bm{X}}\left[\hat{f}_{n,\tilde{k}}(X_{i_0})\right]-f(x_0) \right| & \leq \max_{q \in [\tilde{k}]}\left\lbrace \left| f\left(X_{\tau_{n,q}(X_{i_0})}\right)-f(x_0)\right|\right\rbrace\\ & \leq \max_{q \in [\tilde{k}]}\left\lbrace \holderConstant\cdot \dist\left(x_0,X_{\tau_{n,q}(X_{i_0})}\right)^{\holderExponent}  \right\rbrace\\
& \leq \holderConstant \cdot \left( 3 \cdot \xi\right)^{\holderExponent} \leq 3 \cdot   {\holderConstant}^{\frac{\dimensionExponent}{2\holderExponent+\dimensionExponent}} \cdot\left( \frac{\log(4n/\delta)}{\densityFunction(x_0)\cdot n} \right)^{\frac{\holderExponent}{2\holderExponent+\dimensionExponent}}.
\end{align*}
Combining with (\ref{conditionalExpectationApplicationBoundInMaxThmPf}) we deduce that
\begin{align*}
\hat{M}_{n,\delta}(f)  &\geq \hat{f}_{n,k}(X_{i_0})-f(x_0)-\sqrt{\frac{\log(4n/\delta)}{\tilde{k}}}\\
& \geq \E_{\bm{Z}|\bm{X}}\left[\hat{f}_{n,\tilde{k}}(X_{i_0})\right] -4\cdot \sqrt{\frac{\log(4n/\delta)}{4\tilde{k}}}\\
& \geq f(x_0) - 3 \cdot   {\holderConstant}^{\frac{\dimensionExponent}{2\holderExponent+\dimensionExponent}} \cdot\left( \frac{\log(4n/\delta)}{\densityFunction(x_0)\cdot n} \right)^{\frac{\holderExponent}{2\holderExponent+\dimensionExponent}} -4\cdot \sqrt{\frac{\log(4n/\delta)}{4\tilde{k}}}\\
& \geq f(x_0) - 7 \cdot   {\holderConstant}^{\frac{\dimensionExponent}{2\holderExponent+\dimensionExponent}} \cdot\left( \frac{\log(4n/\delta)}{\densityFunction(x_0)\cdot n} \right)^{\frac{\holderExponent}{2\holderExponent+\dimensionExponent}},
\end{align*}
where the final inequality follows from the lower bound in (\ref{tildeKBoundForMaxThm}). This gives the lower bound in (\ref{toProveInMaxThmBound}). To prove the upper bound we observe that for each $i \in [n]$ we have $\E_{\bm{Z}|\bm{X}}\left[\hat{f}_{n,k}(X_i)\right] = \sum_{q \in [k]}f\left(X_{\tau_{n,q}(X_i)}\right) \leq M(f)$. Hence, the upper bound in (\ref{toProveInMaxThmBound}) follows from (\ref{conditionalExpectationApplicationBoundInMaxThmPf}). This completes the proof of (\ref{tildeKBoundForMaxThm}). Letting $\epsilon \rightarrow 0$ we deduce Theorem \ref{funcMaxThm}.
\end{proof}
\begin{corollary}\label{fastLimitsMaxThmCorollary} Suppose that $f$ satisfies the H\"{o}lder assumption with parameters $(\holderExponent, \holderConstant)$ and $\marginalDistribution$ satisfies the minimal mass assumption with parameters $(\dimensionExponent, \densityFunction)$. Suppose further that for some $\fastLimitsExponent \in (0,\infty]$, $\fastLimitsConstant \geq 1$ and $\fastLimitsThreshold \in (0,1)$, for each $\epsilon \in (0,\fastLimitsThreshold)$ we have $\sup_{x\in \suppMarginalDistribution}\left\lbrace f(x): \densityFunction(x)>\epsilon \right\rbrace \geq M(f)-\fastLimitsConstant \cdot \epsilon^{\fastLimitsExponent}$. Then, for each $n \in \N$ and $\delta \in (0,1)$ with probability at least $1-\delta$ over $\sample_f$,
\begin{align*}
\left|  \hat{M}_{n,\delta}(f) - M(f)\right| \leq 8 \cdot\left(\holderConstant^{\dimensionExponent/\holderExponent}\cdot (\fastLimitsConstant/\fastLimitsThreshold) \right)^{\frac{\holderExponent}{2\holderExponent+\dimensionExponent}}\cdot\left( \frac{\log(4n/\delta)}{ n} \right)^{\frac{\fastLimitsExponent \holderExponent}{\fastLimitsExponent(2\holderExponent+\dimensionExponent)+\holderExponent}}.
\end{align*}
\end{corollary}
\begin{proof}
Combine Theorem \ref{funcMaxThm} with $\sup_{x\in \suppMarginalDistribution}\left\lbrace f(x): \densityFunction(x)>\epsilon \right\rbrace \geq M(f)-\fastLimitsConstant \cdot \epsilon^{\fastLimitsExponent}$ and \[\epsilon = \min \left\lbrace \fastLimitsThreshold, \left( \holderConstant^{\dimensionExponent}/\fastLimitsConstant^{2\holderExponent+\dimensionExponent}\right)^{\frac{ 1}{\fastLimitsExponent(2\holderExponent+\dimensionExponent)+\holderExponent}} \cdot \left( \frac{\log(4n/\delta)}{ n} \right)^{\frac{ \holderExponent}{\fastLimitsExponent(2\holderExponent+\dimensionExponent)+\holderExponent}}\right\rbrace.\]
\end{proof}

==> plan.tex <==
Order:



1. Intro

- Problem set up

- Related work

- Scott & MPE

- Main achievements

Minimax bound
Lower bounds
Function maximisation


- Outline of paper...


3. Statistical setting: Asymmetric label noise


- Define excess risk
- Define Bayes classifier

* Most labels are correct


Identifying unknown label noise..

- Emphasise unknown label noise

- Point towards range assumption...

* Range assumption


Standard assumptions


* Tsybakov's margin assumption.. (TMA)
- Emphasise different to label noise

* Holder regression function
- Our approach will be adaptive..

* Minimal mass assumption 


4. Densities bounded away from zeroes

Emphasise just for contrast...

Assumption: Bdd away from 0 assumption...

Statement of thm





Pf..
Lower bound A \& T
Upper bound in Sec ...

Short-comings - something about Gaussian measures...

5. Flexible densities


* Tail condition (TA)

Correspond to Gadat..

Examples


* Quantitative range assumption
* Marginal districing give standard Menon's range assumption..
- explain how this gives rise to identifiability...
- but not enough...
- state assumption quantitative range assumption..
. compare with Menons $\&$ Scott's. Note that its weaker than attainment! (ie. Scott's assumption)
- cite recent work on MPE

- Emphasise threshold regime..

Recompare with literature
- Gadat's work.. -Emphasise differences in the upper bound (unknown smoothness, unknown density.
    - Log factor weaker (estimating noise factor)
    - Threshold changes the logarithmic factor...
-Canning's work on non-shifted decision boundary). 


- Scott et al.s work - parametric setting.. Fast rates would be possible.. Assumptions loosely correspond to $\tau = \infty$..


- Structure of the proof / Rest of the paper..

6. KNN regression with the locally 

Main theorem for arbitrary $k$

C \& D type lemma... (simple form with single $k$)
Pf. in appendix

Lepski... corollary


7. Estimating the maximum of a function

- State why (ie. link to quantitative range assumption)

- State new setting  and then the problem

- State intuition...

- State algo - influenced by UCB methods

- State bound


8. An algorithm with a high probability upper bound



9. Lower bound 1: Known label noise

10. Lower bound 2: Unknown label noise

11. Discussion



Appendix:

1. high prob measure of ball around k-nn..
2. Concentration eq. for reg func around cond. expectation..








- Move regular KNN stuff to an appendix
- Reformulate into a) Bayes error can be phrased in terms of corrupted regression function \& shifted decision boundary...




?? Why metric spaces - manifolds \& explains what is conceptually important.




To do:

1. Complete the two lower bounds
2. Complete the minimax theorem statement (with constants etc.) and statement of upper bound
3. Fix proof of max location
4. Put in reverse Pinsker's inequality
5. Move proof of K-NN Regression to its own appendix
6. Print out and fix notation
7. Sort intro...
8. Use ``measureable' with respect to sample notation of Gadat..



ORDER components correctly ????!!! Tau bit first...???


Gadat bounds high prob???



INTRO

IMPORTANCE of 
a) label noise: Why important?
Asymmetric label noise
PU data..

- Blanchard \& Menon assumption
Known noise probabilities..
Unknown - Scott \& Kernel
Adaptive estimation of the mode of a multivariate density.
Mixture proportion estimation via kernel embeddings of distributions
-. Learning from
Corrupted Binary Labels via Class-Probability Estimation. 

ErM -A Theory of Learning with Corrupted Labels



- Finite sample rates require geometric assumptions either balls (Scott) or seperability on Hilbert space.



b) Why non-parametric view..
A general distribution dependent theory account..
Should include unbounded domains
Gadat


c) Interaction is interesting because extrema need not be attained..

Key conclusion:
Minimax rate depends on the speed at which extrema is reached..

An adaptive algorithm with a high probability upper bound. + Complementary lower bound (equal up to logarithmic factors)..

Two component sub lower bounds
1. is more standard (but non-integer d & satisfy tail properties)
2. two distributions..

(python figure if time permits...)



Differences with Gadat:
Dealing with asymmetric label noise


Emphasise adaptivity:

Regression component:


1) local density as well as H\"{o}lder exponent and dimension
- Contrast with Gadat in terms of using prior knowledge of the local density
- A metric space setting.

2) Less restrictive than 

- Contrast with Garg \& Kopotufe.
*G \& K is also an abstract metric space..
*Less restrictive as it doesn't require an upper bound on the covering number... (union bound over points).
* We have results for a fixed point rather than uniform.. (used via the Markov inequality).


Max est component:

Compare with mode estimation 
Jiang 
1) Strong assumptions on 1) local maximum with a negative define Hessian..
2) Uniform lower bound on density
- a genuine problem - means we can't simply use KNN estimates.
3) Dasgupta \& Kpotufe require twice differentiable function

Active problem of $\X$-armed bandit..

* Interesting in its own right...

INSIGHT - Bias always points in one way...






Why a metric space setting:

1) Manifolds..
Density level set estimation on manifolds with dbscan - For manifold's 
2) Conceptual clarity..

- put this in the intro???


Assumptions - Gadat table with different distributions..


To do:


5. Clean up assumptions sec...
8. Sort out intro to algo somewhere....?? - Maybe after lower bound...
6. Write discussion.
7. Intuition for upper bound
8. Change unbounded to non-compact ...
9. Sort out sections one by one ...


Should we allow infinite $\tau$??? - Probably not



==> technicalLemmasInTheProofOfTheLowerBound.tex <==

\section{Technical lemmas in the proof of the lower bound}\label{technicalLemmasInLBPf}


\begin{comment}


The proof of the lower bound utilised the following variant of Fano's lemma due to Birge a proof of which may be found in \cite{birge2001new}, which we learnt from \cite{audibert2004classification}.

\begin{lem}\label{birgesVersionOfFanosLemma} Given a finite family $\mathcal{S}$ consisting of probability measures on a measureable space $\left(\mathcal{Z},\Sigma\right)$ and a random variable $Z$ with an unknown distribution in the family, then we have
\begin{align*}
\inf_{\hat{T}}\left\lbrace \sup_{{\Prob}_Z\in \mathcal{S}}\left\lbrace \Prob_Z\left[\hat{T}(Z) \neq \Prob_Z\right]\right\rbrace\right\rbrace \geq \min\left\lbrace 0.36,1- \inf_{\Prob_Z \in \mathcal{S}}\left\lbrace \sum_{\tilde{\Prob}_Z \in \mathcal{S}} \frac{\kullbackLeiblerDivergence\left(\Prob_Z,\tilde{\Prob}_Z\right)}{\left|\mathcal{S}\right|\log\left|\mathcal{S}\right|}  \right\rbrace\right\rbrace,
\end{align*}
where the infimum is taken over all measureable (possibly randomised) estimators $\hat{T}:\mathcal{Z}\rightarrow \mathcal{S}$.
\end{lem}

\end{comment}

\begin{proof}[Proof of Lemma \ref{propertiesCheckLemmaForUnknownNoiseLB}] We check each property in turn.

\noindent Property \ref{classConditionalNoiseAssumption} follows immediately from the construction of $\Prob^{\twoMeasuresUnknownNoiseDistIndex}$ together with the fact that $\Delta <1/6$, so each $\probFlipFrom[j]^{\twoMeasuresUnknownNoiseDistIndex}<1/4$.

\noindent Property \ref{marginAssumption} follows from the fact that since $\Delta<1/6$, we have $\left|\regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(x)-1/2\right| \geq 1/3$ for $x \neq c$ and 
$\left|\regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(c)-1/2\right|\geq \Delta/4$. Property \ref{holderAssumption} follows from the fact that the only two distinct points $x_0, x_1$ with $\dist(x_0,x_1)<1$ are $a$ \& $b$ with $\dist(a,b)=r$ and $\left|\regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(a)-\regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(b)\right|\leq \Delta$.

\noindent Property \ref{minimalMassAssumption} follows from the fact that  $\marginalDistribution$ is defined by $\marginalDistribution(\{a\}) = \volA$, $\marginalDistribution(\{b\}) = 1/3$, $\marginalDistribution(\{c\}) = \volC$, $\marginalDistribution(\{d\}) = 2/3-\volA-\volC$ and $\densityFunction:\X \rightarrow (0,1)$ by $\densityFunction(a)=\densityA$, $\densityFunction(c) = \volC$ and $\densityFunction(b) =\densityFunction(d)=1/3$. In particular, for $x \neq a$ we have for $\tilde{r} \in (0,1)$ \[\marginalDistribution(B_{\tilde{r}}(x))\geq \marginalDistribution(\{x\}) \geq \densityFunction(x) \geq  \densityFunction(x) \cdot {\tilde{r}}^d.\]
On the other hand, for $x = a$ there are two cases. If ${\tilde{r}} \in (r,1)$ then \[\marginalDistribution(B_{\tilde{r}}(a))\geq \marginalDistribution(\{b\}) \geq 1/3 \geq \densityA \cdot {\tilde{r}}^{\dimensionExponent}=\densityFunction(a)\cdot {\tilde{r}}^{\dimensionExponent} \] since $\densityA <1/6$. If ${\tilde{r}}\leq r$ then $\marginalDistribution(B_{\tilde{r}}(a)) \geq \marginalDistribution(\{a\}) = \volA \geq \densityA \cdot r^d \geq \densityFunction(a)\cdot {\tilde{r}}^{\dimensionExponent}$.

\noindent Property \ref{tailAssumption} requires three cases. If $\epsilon \in [\max\{\densityA, \volC\},1/3)$ then we have
\[\marginalDistribution\left(\{x \in \X: \densityFunction(x)<\epsilon\}\right) =\marginalDistribution\left(\{a,c\}\right) = \volA+\volC \leq 2\max\{\densityA,\volC\} \leq \tailsConstant \cdot \epsilon^{\tailsExponent}.\]
If $\epsilon \in [\min\{\densityA, \volC\},\max\{\densityA, \volC\})$ then we take $x_0 \in \{a,c\}$ with $\densityFunction(x_0) = \min_{x \in \X}\{\densityFunction(x)\}$. Since $\volA \leq \densityA$ we have 
\[\marginalDistribution\left(\{x \in \X: \densityFunction(x)<\epsilon\}\right) =\marginalDistribution\left(\{x_0\}\right) \leq \densityFunction(x_0) = \min\{\densityA, \volC\}\leq \epsilon \leq \tailsConstant \cdot \epsilon^{\tailsExponent}.\]
Finally, for  $\epsilon \in (0,\min\{\densityA, \volC\})$ we have $\marginalDistribution\left(\{x \in \X: \densityFunction(x)<\epsilon\}\right)=0$.

\noindent Property \ref{quantitativeRangeAssumption} requires us to consider two cases. If $\epsilon \in [w, \fastLimitsThreshold)$ then since $\densityFunction(b) =\densityFunction(d)=1/3>\epsilon$ and for both $\twoMeasuresUnknownNoiseDistIndex \in \{0,1\}$ we have $\regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(b) \geq 1-\Delta$ and $\regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(d)=0$ we have 
\begin{align*}
\max\left\lbrace \inf_{x \in \suppMarginalDistribution}\left\lbrace \regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(x): \densityFunction(x) >\epsilon \right\rbrace, \inf_{x \in \suppMarginalDistribution}\left\lbrace 1-\regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(x): \densityFunction(x) >\epsilon \right\rbrace\right\rbrace \leq \Delta \leq \fastLimitsConstant \cdot \epsilon^{\fastLimitsExponent}.    
\end{align*}
On the other hand, if $\epsilon \in (0,w)$ then since $\densityFunction(a)=w$ and $\regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(a)=1$, and $\regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(d)=0$ we have
\begin{align*}
\max\left\lbrace \inf_{x \in \suppMarginalDistribution}\left\lbrace \regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(x): \densityFunction(x) >\epsilon \right\rbrace, \inf_{x \in \suppMarginalDistribution}\left\lbrace 1-\regressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(x): \densityFunction(x) >\epsilon \right\rbrace\right\rbrace= 0 \leq \fastLimitsConstant \cdot \epsilon^{\fastLimitsExponent}.    
\end{align*}




\end{proof}





\paragraph{Proof of Lemma \ref{KLBoundOnPairOfProductDistributionsLemma}} We shall show that $\kullbackLeiblerDivergence\left(\left(\noisy[\Prob]^{0}\right)^{\otimes n},\left(\noisy[\Prob]^{1}\right)^{\otimes n}\right)\leq n\cdot \volA \cdot (3\Delta/2)^2$. The proof that\\ $\kullbackLeiblerDivergence\left(\left(\noisy[\Prob]^{1}\right)^{\otimes n},\left(\noisy[\Prob]^{0}\right)^{\otimes n}\right)\leq n\cdot \volA \cdot (3\Delta/2)^2$ is similar. Recall that for each ${\twoMeasuresUnknownNoiseDistIndex}\in \{0,1\}$ we let $\noisy[\Prob]^{\twoMeasuresUnknownNoiseDistIndex}$ denote the marginal distribution of $\Prob^{\twoMeasuresUnknownNoiseDistIndex}$ over pairs $(X,\noisy[Y])$ consisting of a feature vector $X \sim \X$ and a corrupted label $\noisy[Y]\in \Y$. We can compute the corrupted regression functions $\noisyRegressionFunction^{\twoMeasuresUnknownNoiseDistIndex}(x)= \Prob^{\twoMeasuresUnknownNoiseDistIndex}[\noisy[Y]|X=x]$ for ${\twoMeasuresUnknownNoiseDistIndex}\in \{0,1\}$ by applying (\ref{writingCorruptedRegressionFunctionInTermsOfRegressionFunctionEq}). Since $\probFlipZeroToOne^0=0$ and $\probFlipOneToZero^0=1/4$ we have $\noisyRegressionFunction^0(x) = (3/4)\cdot \regressionFunction^0(x)$ for all $x \in \X$. On the other hand, since $\probFlipZeroToOne^1=0$ and $\probFlipOneToZero^1=(1+3\Delta)/4$ we have $\noisyRegressionFunction^1(x) =(3/4)\cdot(1-\Delta)\cdot \regressionFunction^1(x)$ for all $x \in \X$.

We begin by bounding the  Kullback Leibler divergence between $\noisy[\Prob]^0$ and $\noisy[\Prob]^1$ using the fact that $\marginalDistribution(\{a\})=\volA$  and $\noisyRegressionFunction^0(x)=\noisyRegressionFunction^1(x)$ for $x \in \X \backslash \{a\}$,
\begin{align*}
\kullbackLeiblerDivergence\left(\noisy[\Prob]^{0},\noisy[\Prob]^{1}\right)& = \sum_{x \in \X}\sum_{y \in \Y} \noisy[\Prob]^0\left[X = x\hspace{2mm}\&\hspace{2mm}\noisy[Y]=y \right] \log \left(\frac{\noisy[\Prob]^0\left[X = x\hspace{2mm}\&\hspace{2mm}\noisy[Y]=y \right]}{\noisy[\Prob]^1\left[X = x\hspace{2mm}\&\hspace{2mm}\noisy[Y]=y \right]}\right)\\
& = \sum_{x \in \X} \marginalDistribution(\{x\}) \left( (1-\noisyRegressionFunction^0(x)) \log\left( \frac{1-\noisyRegressionFunction^0(x)}{1-\noisyRegressionFunction^1(x)}\right) + \noisyRegressionFunction^0(x)\log\left( \frac{\noisyRegressionFunction^0(x)}{\noisyRegressionFunction^1(x)}\right)
\right)\\
& = \volA \cdot \left( (1-\noisyRegressionFunction^0(a)) \log\left( \frac{1-\noisyRegressionFunction^0(a)}{1-\noisyRegressionFunction^1(a)}\right) + \noisyRegressionFunction^0(a)\log\left( \frac{\noisyRegressionFunction^0(a)}{\noisyRegressionFunction^1(a)}\right)
\right)\\
& \leq \volA \cdot \frac{\left(\noisyRegressionFunction^0(a)-\noisyRegressionFunction^1(a)\right)^2}{\min \left\lbrace \noisyRegressionFunction^0(a), (1-\noisyRegressionFunction^0(a)),\noisyRegressionFunction^1(a), 1-\noisyRegressionFunction^1(a)\right\rbrace}\leq  \volA \cdot (3\Delta/2)^2.
\end{align*}
The second to last inequality follows from the reverse Pinsker's inequality \cite[Lemma 6.3]{csiszar2006context}. The final inequality follows from the fact that $\noisyRegressionFunction^0(a) = 3/4$ and $\noisyRegressionFunction^0(a)=(3/4)\cdot (1-\Delta)$. Given that  $\left(\noisy[\Prob]^{\twoMeasuresUnknownNoiseDistIndex}\right)^{\otimes n}$ consists of $n$ independent copies of $\noisy[\Prob]^{\twoMeasuresUnknownNoiseDistIndex}$ for $\twoMeasuresUnknownNoiseDistIndex \in \{0,1\}$ we deduce that \[\kullbackLeiblerDivergence\left(\left(\noisy[\Prob]^{0}\right)^{\otimes n},\left(\noisy[\Prob]^{1}\right)^{\otimes n}\right)= n \cdot \kullbackLeiblerDivergence\left(\noisy[\Prob]^{0},\noisy[\Prob]^{1}\right) \leq n\cdot \volA \cdot (3\Delta/2)^2.\]

\QEDA

